From Regulation to Support: Centering Humans in Technology-Mediated Emotion Intervention in Care Contexts

Enhancing emotional well-being has become a significant focus in HCI and CSCW, with technologies increasingly designed to track, visualize, and manage emotions. However, these approaches have faced criticism for potentially suppressing certain emotional experiences. Through a scoping review of 53 empirical studies from ACM proceedings implementing Technology-Mediated Emotion Intervention (TMEI), we critically examine current practices through lenses drawn from HCI critical theories. Our analysis reveals emotion intervention mechanisms that extend beyond traditional emotion regulation paradigms, identifying care-centered goals that prioritize non-judgmental emotional support and preserve users' identities. The findings demonstrate how researchers design technologies for generating artificial care, intervening in power dynamics, and nudging behavioral changes. We contribute the concept of "emotion support" as an alternative approach to "emotion regulation," emphasizing human-centered approaches to emotional well-being. This work advances the understanding of diverse human emotional needs beyond individual and cognitive perspectives, offering design implications that critically reimagine how technologies can honor emotional complexity, preserve human agency, and transform power dynamics in care contexts.

==> Acut.tex <==
before methods

\section{intro}

HCI and CSCW scholars have been increasingly devoted to the emotional wellbeing in workplaces, everyday contexts, study. Emotional work is especially important in various care context such as chronical diseases, mental health, vulnerable populations such as children and elder adults. 
Researchers working in the emerging field of emotion AI, aiming to recognize, modify, and regulate individuals' emotions. Such practices are based on the adopted of "emotion regulation" directly from psychology and developed various technologies, However, traditional approaches to emotion regulation have often focused on the modification or suppression of emotions, reflecting a bias towards "correcting" emotional responses. This perspective has been criticized for failing to acknowledge that many emotions originate from societal oppression, normative assumptions, and expectations rooted in social norms \cite{ahmed_cultural_2014}. 

However, technologies for emotion regulation has been criticized by individual emotional experiences are subject to surveillance and regulation by monitoring, sensing, and tracking machines \cite{boyd_automated_2023}, intruding into people's most sensitive and private spaces \cite{choe_emotion_2023}. 
Previous scholars have noted that digital tools may serve as a new vector for colonialism and oppression, advocating for justice- \cite{chordia_social_2024} and ethics-oriented research. 
\textcite{pendse_treatment_2022} untangled the coloniality of digital mental health tools in continuing and expanding the historically oppressive and Western-established paradigm of treatment-centered psychological approaches. This paradigm may contribute to stigmas around diseases and force the marginalization of certain communities by labeling them as ``ill''.
%Treatment-centered research is based on psychological theories such as Gross's emotion regulation process model \cite{gross_emotion_1998} and cognitive behavioral therapy which may sustain the coloniality through technical design. 

Feminism has a foundational contribution to the social and experiential understanding of emotion in comparison to biology-determined and categorical emotions. We leverage feminist perspectives on psychology and emotions to chart the dimensions of "emotional support" (in comparison to the psychological term, "emotion regulation"?) to challenge traditionally male-dominated knowledge creation about mental health and psychological understanding of human emotions. A feminist approach to emotional support emphasizes acceptance and validation rather than correction, aligning with the real-world experiences of individuals facing systemic challenges \cite{hooks_feminism_2000}. We investigate how current technology-supported emotion interventions are designed and how they influence gendered care work, primarily performed by women. 

Inspired by critical reflections on the potential harms of digital tools to human emotions, feelings, identities, and experiences, this work aims to reimagine technology's role in care-centered emotional support. The research questions of this work include:


Specifically, we conducted a systematic literature review on the ACM digital library and investigated how existing technology-mediated emotional support interventions understand and intervene in human emotions in health contexts.
However, the wide application of TMEI also draws criticism from various scholars. Andalibi \cite{andalibi_human_2020} challenges the fundamental premise that algorithms can accurately identify objective 'ground truth' emotional states, arguing that emotional experiences are inherently subjective and contextually variable. Similarly, \textcite{10.1145/3442188.3445939} question the validity of algorithmic emotion categorization, highlighting how conceptualizations of emotions differ substantially across individuals and contexts. 

More pointed concerns emerge from researchers like Pendse et al. \cite{pendse_treatment_2022} who caution against the problematic tendency of these technologies to prioritize "correcting" emotional responses through modification or suppression. For example, systems that prompt users to "cheer up" when detecting sadness or that suggest breathing exercises to "fix" detected anxiety may implicitly frame certain emotional states as undesirable or abnormal rather than as valid responses to life circumstances. This critique is extended by \textcite{10.1145/3544548.3581480}, who critically examines how curative technological approaches can place unreasonable expectations on disabled users, potentially reinforcing harmful normative assumptions about emotional expression.
Critics further argue that digital tools may serve as a new vector for colonialism and oppression \cite{chordia_social_2024}, risking the subjection of individual emotional experiences to surveillance through monitoring, sensing, and tracking machines \cite{choe_emotion_2023}. 
%delineated a "counterventional" framework that foregrounds the undue burden of improvement placed on the disabled user by "curative" technologies; they call for privileging the desires of participants who serve as cultural informants rather than research subjects

In response, a growing body of work in HCI has advocated for justice- and ethics-oriented research \cite{chordia_social_2024}, recentering the intentions and needs of the people that technologies are intended to support. Researchers have called for design practices beyond a categorical understanding of emotions as biologically determined and universally expressed \cite{kitson_supporting_2024, petr_slovak_designing_2023}. Instead, they advocate for technologies that honor individuals' stories through approaches that recognize emotions as co-constructed with others \cite{10.1145/3610073, 10.1145/3512939} and embodied through physical sensations \cite{10.1145/3064663.3064697, 10.1145/3491102.3502135, 10.1145/3490149.3501326}. For example, Lazar et al. \cite{10.1145/3359187} expanded the scope of emotion expression by emphasizing non-verbal communication essential for disabled people with health-related communication barriers. Similarly, researchers have sought to amplify the understanding of emotional needs by incorporating voices from historically underrepresented populations. For instance, \textcite{bhattacharjee_whats_2023} documented Indian people's avoidance of helpline-delivered talk therapy that is rooted in Western psychology, highlighting the cultural specificity of emotional interventions.\subsection{The detailed version of harms of TMEIs}


\subsection{Psychological foundation of Emotion and Emotion Regulation}
Psychological knowledge about emotion originated in the late 19th century, influenced in particular by the work of William James \cite{james1948emotion}, setting foundations for the cognitive factors and a maladaptive treatment-focused approach to emotion regulation \cite{kovacs1978maladaptive}.

\subsubsection{Biological determinism}
% Early work in psychology distinguished "affect" from "emotion". Charles Darwin claimed ``affect'' was determined by individual's biological responses and physiological changes \cite.\cite{tomkins2014affect}. James Russell, a prominent figure in emotion research, conceptualized core affect along two dimensions of neural sensations: valence and arousal. Valence denotes a global assessment of pleasure and displeasure, while arousal varies in levels of activation and deactivation \cite{russell1989affect}. Further expanding on this biological perspective, Ekman proposed the Basic Emotions Theory, which posits a universal set of six discrete, mutually exclusive emotions: anger, disgust, fear, joy, sadness, and surprise \cite{ekman1992there}. This theory has been influential, with abundant research adopting these predefined categories of emotions for recognition, surveillance, and intervention purposes.

Such understanding of emotions serves as the foundation of the field of Affective Computing, pioneered by Picard (1995) which aims to enhance human-technology interaction through emotion-sensitive systems \cite{}, focusing on developing technologies that can recognize, interpret, and simulate human emotions.
The biological perspective on emotion has only recently been critically examined by those working in Human-Computer Interaction (HCI) studies about Emotion AI. These researchers argue that "emotions are constructed by individuals within social contexts, shaped by personal and socio-cultural differences rather than universally expressed; emotional experiences are structured from multiple overlapping, fundamental affective dimensions instead of discrete categories" \parencite{roemmich_emotion_2024}. This shift in understanding presents both challenges and opportunities for the field of Emotion AI, as it grapples with integrating more nuanced, socially informed approaches to emotion in its technological applications. The evolving perspective necessitates a balance between innovation and a deeper understanding of the multidimensional nature of human emotions.

\subsubsection{Maladaption centered Emotion Regulation}
Emotion regulation has emerged as a central field in psychology, focusing on the modification of people's affect and emotional status. James Gross's Process Model \cite{gross_antecedent-_1998} has formed the foundation of emotion regulation research, suggesting five strategies: situation selection, situation modification, attentional deployment, cognitive change, and response modulation. These strategies aim to alter responses in experiential, behavioral, and physiological domains.
Researchers have widely drawn on this framework to examine maladaptive strategies in relation to clinical disorders. Three strategies are commonly theorized to protect against psychopathology: reappraisal, problem-solving, and acceptance. Conversely, three strategies consistently associated with increased risk of psychopathology are: suppression (of expression and thought), avoidance, and rumination \citep{aldao_emotion-regulation_2010, sheppes_emotion_2015}.

However, this strategy-based framework, which centers on the modification of emotional experiences, falls short of articulating the multifaceted nature of emotion regulation. In response to these limitations, Gratz and Roemer adopted a more comprehensive lens, focusing on overall deficits in emotional functioning to delineate dimensions of emotion regulation. Their approach involves awareness, clarity, and acceptance of emotions, the ability to control impulses and engage in goal-directed activities in the face of negative emotions, as well as the capacity to utilize appropriate strategies to flexibly modulate rather than eliminate emotional responses based on situational demands. According to this perspective, individuals are considered to have emotion dysregulation if they show a deficiency in any of these aspects \cite{sloan_emotion_2017}.



\subsection{Feminist Psychology}
%They posit that emotions are not irrational or opposed to reason, but are instead valuable sources of knowledge and insight. Generally, emotional responses have been conceived of as partially non-rational, and this historically has carried with it a view of emotional responses as a sign of loss of control, which has manifest itself in stereotypical portrayals as rationality being masculine and emotionality being more feminine. 
%Feminist psychology emerged as a transformative force within the field, challenging traditional paradigms and introducing new perspectives on human behavior and experience \cite{stewart2006feminist}.  \textcite{parlee1979psychology} and \textcite{vaughter1976psychology} emphasized the potential for feminism to bring about fundamental changes in psychology, not just in terms of studying women but in reconceptualizing the entire discipline.  The development of feminist psychology aims to address the historical marginalization of women's experiences and perspectives in psychological research and theory. Feminist psychology has since evolved to encompass a wide range of theoretical approaches and methodologies, united by a commitment to understanding the impact of gender, power dynamics, and social contexts on psychological processes \cite{gorton2007theorizing}. 

Feminist psychology emerged as a transformative force within the field, challenging traditional paradigms and introducing new perspectives on human behavior and experience \cite{stewart2006feminist}. As \textcite{vaughter1976psychology} articulated, feminist psychology aims "to change the structure of the belief system of science to construct a psychology of human behavior" (p. 146). This approach has had profound implications for the study and understanding of emotions.


Psychologists have noted the interdisciplinary space where feminism contributes to affect theory, often with contradictory and oppositional views. However, there is a shared interest in how "feeling is negotiated in the public sphere and experienced in the body" \cite{goodley_feeling_2018}. The development of feminist psychology aims to address the historical marginalization of women's experiences and perspectives in psychological research and theory. \textcite{parlee1979psychology} and \textcite{vaughter1976psychology} emphasized the potential for feminism to bring about fundamental changes in psychology, not just in terms of studying women but in reconceptualizing the entire discipline. 

Feminist psychology has since evolved to encompass a wide range of theoretical approaches and methodologies, united by a commitment to understanding the impact of gender, power dynamics, and social contexts on psychological processes \cite{gorton2007theorizing}. This perspective has been particularly influential in reshaping our understanding of emotions.

Feminist perspectives on emotion offer a nuanced and multifaceted interpretation that challenges traditional views and has significant implications for understanding emotion regulation, including its technological applications. While there isn't a single, unified feminist definition of emotion, a feminist perspective generally views emotions as complex, socially constructed experiences shaped by cultural norms, power dynamics, and individual lived experiences. Emotions are seen as valuable sources of knowledge and insight, deeply connected to bodily sensations and cognitive processes, and influenced by intersecting social identities.

\subsubsection{Emotion as Experiences}
Feminist approaches to emotion challenge traditional dichotomies and offer a more nuanced view of emotional experiences. A key aspect of this perspective is the rejection of the emotion-reason dichotomy that has long dominated Western philosophy and psychology. This dichotomy is evident in neurobiological analyses of emotion experience. Treatments such as Cognitive Behavioral Therapy (CBT) indicate that mental representations of emotion can be linked to psychological situations. These treatments hypothesize that a mental representation of emotion on a particular occasion is a continuously changing stream of consciousness in which core affect evolves, interacts with, and mutually constrains construals of the psychological situation \cite{barrett2007experience, barrett2006emotions}.

The historical divide associating rationality with masculinity and emotion with femininity has been used to devalue women's experiences and perspectives \textcite{jaggar2014love}. In contrast, feminist psychologists argue for a more integrated understanding of emotion and cognition. They posit that emotions are not irrational or opposed to reason, but are instead valuable sources of knowledge and insight. generally, emotional responses have been conceived of as partially non-rational, and this historically has carried with it a view of emotional responses as a sign of loss of control, which has manifest itself in stereotypical portrayals as rationality being masculine and emotionality being more feminine. Feminist theory challenges this dichotomy and suggests value in considering emotions as a source of potential knowledge and insight \cite{barrett2006emotions}.

Embodiment of Emotion. Feminist theories often emphasize the embodied nature of emotions, challenging the Cartesian dualism that separates mind and body. This perspective, as articulated by theorists like \textcite{elizabeth1994volatile}, recognizes the interconnection between physical sensations, cognitive processes, and emotional experiences.

The embodiment of emotion has important implications for understanding how emotions are experienced and regulated. It suggests that emotional experiences are not purely mental phenomena but are deeply connected to bodily sensations and processes. This view encourages a holistic approach to studying and supporting emotional well-being.

\subsubsection{Social Construction of Emotion}
A key tenet of feminist approaches to emotion is the recognition that emotions are socially constructed \cite{frijda2017laws}. Rather than viewing emotions as purely biological or innate phenomena, feminist psychologists argue that emotional experiences are shaped by social and cultural contexts, including societal norms, power structures, and gender roles \textcite{boiger2012construction}. This social constructionist view has important implications for understanding emotional experiences across different cultures and social groups. It suggests that the way we experience and express emotions is not universal but is deeply influenced by our social environment and learned cultural scripts.

Feminist perspectives on emotion emphasize the role of power dynamics and the potential for empowerment through emotional experiences. Emotions are seen not as weaknesses to be controlled or suppressed, but as potential catalysts for personal growth and social change. Intersectionality \cite{crenshaw2013mapping} has become a crucial framework in feminist psychology for understanding emotions. This approach recognizes that emotional experiences are influenced by various intersecting identities such as gender, race, class, and sexuality. An intersectional perspective allows for a more nuanced understanding of how different social positions and power dynamics shape emotional experiences and expressions.



%Feminist theory has contributed significantly to our understanding of emotional labor, particularly in how it is often disproportionately expected of women and undervalued in society. Arlie Hochschild, who coined the term "emotional labor" in 1983, described it as the process of managing feelings and expressions to fulfill the emotional requirements of a job. Feminist scholars have since expanded this concept to include unpaid emotional work in personal relationships and caregiving roles.

\section{UX related Cut}
\subsubsection{User Experience Goals}
% Collapse categories between the two --> hint at qual's advantage in unveiling richer insights, the "why")
% ( n = 13 include both quant and qual: 11 on engagement, 13 touched upon affective)

% "Many standardized instruments that are well established in usability research (such as questionnaires) cannot be used due to the cognitive impairments of the target group...wearable sensors poorly accepted...evoke anxiety..." - to justify use "observation' to assess intervention outcomes

Our review identified user engagement as the most prevalent user experience goal across studies, which was operationalized across cognitive, affective, and behavioral domains in relation to unique technology affordances. Overall,  design solutions aimed to stimulate and sustain users' active involvement as the prerequisite to realize the interventions' full potential. For instance, studies demonstrated the duration and consistency of user engagement via logged data \cite{10.1145/3329189.3329209} and field observations \cite{10.1145/3064663.3064697, 10.1145/3154862.3154929, 10.1145/3490149.3501326}, and analyzed sensory interactions (e.g., touch, gaze) as the behavioral evidence of involvement  \cite{10.1145/3173574.3174069}. 

Many studies also tapped into the hedonic, affective components of user engagement (n = 13), such as enjoyment, playfulness, and the sense of reward during intervention, as proxy for users' intrinsic interests in exploring their emotions \cite{10.1145/3154862.3154929, 10.1145/3130943, 10.1145/3575879.3575997}. Three studies showed that the overall experience of interacting with the systems was pleasant and satisfying, confirming that the functions and interfaces met users' expectations \cite{10.1145/3628516.3655820,10.1145/2544104, 10.1145/3434073.3444669}. In addition, four studies with companion robots and embodied toys highlighted users' socio-emotional responses towards the intervention devices \cite{10.1145/3491102.3502130, 10.1145/3660244, 10.1145/3490149.3501326,10.1145/3173574.3174069}. Two studies that evaluated perceived naturalness, immersiveness, and realism as indicators for states of absorption showed that the elderly often could not differentiate the virtual world from reality  \cite{10.1145/3154862.3154929} or forgot the artificial nature of embodied agents \cite{10.1145/2544104} as they became more engaged in interventions. 

% as indicators for states of absorption to gauge how users perceived the role of technologies in their care environments. Of note, the elders with dementia...perception of virtuality vs. reality

% NOTE: elderly hard to differentiate reality & virtual world (example for unique user needs/ requirment, too immersive can induce uncanny vally or unease certain populations)
% "The experiment revealed that TACO created pleasant, engaging interactions with children, however the tests were not sufficient to show a therapeutic effect. As such, we cannot yet claim that that TACO can positively affect the mood or wellbeing of children."

% "Embodying Care: Naturalness (elderly) : "The physical embodiment of a baby-like face and human-like multimodal attributes facilitates natural interaction with older people who \textbf{seem to forget} they are actually interacting with \textbf{technological} device."
% Activating...acqurium (PwD): "Perception of virtuality vs reality: Depending on their state of dementia, the perception between virtuality and reality varied. In later stages, residents seemingly couldn’t distinguish the virtually generated effect from the real one: In a group session, one PwD tried to collect the fish with both hands indicating that she perceived the fish as real animals. To the best of our knowledge, this has not been observed before.

Regarding pragmatic aspects of user experience, studies assessed perceived usability (n = 6), usefulness (n = 3), feasibility (n = 3) of proposed design solutions, mainly through post-study surveys and interviews. Such efforts to create positive impressions were motivated by the hope to translate this halo effect into further engagement, as catalyst for interventions' efficacy. While most users found intervention devices and systems easy to use and helpful in their ER attempts, some reported challenges of consistent engagement with the technologies for them to be effective \cite{10.1145/3610073, 10.1145/3479561}; one study noted specific usability barriers that stem from physical and cognitive demands during treatment procedures \cite{10.1145/3415183}. Three studies also sought functional feedback from stakeholders other than end-users themselves (e.g., therapists, parents, school aides) \cite{10.1145/3628516.3655820, 10.1145/3575879.3575997, 10.1145/2809915.2809917}, one of the which showed mixed sentiment towards usability between care receivers and caregivers (e.g., students found the system simple to use while therapists considered the user flow needed improvement) \cite{10.1145/3628516.3655820}.




% other feasiblity findings"?
% Usability ( n = 6)
% 2 x Acceptability, 3 x Feasibility, 7 x useful/helpful (not purely qual)
% Expert eval that uncovered usability issues (e.g., MoodGem)

% fallout after initial adoption
% ...claimed that the lack thereof could undermine efficacy of interventions 

%ARCADIA: A Gamified Mixed Reality System for Emotional Regulation and Self-Compassion 
%\textbf{UEQ}: system usability,  user engagement 
%(found to be motivating, innovative and easy to use.)

%MoodShaper VR supports management of neg emo
%\textbf{UEQ}-S: pragmatic (usability and utility) & hedonic (joy and stimulation) qualities. 
%"...determine if the interventions are user-friendly and enjoyable,  
% --> as low scores could undermine the effectiveness of the ER interventions."
%\textbf{UES-SF}:  user engagement with the interventions...
%scores for aesthetic appeal, focused attention, perceived usability, reward factor
%--> "Higher values indicate greater perceived engagement and active involvement, potentially fostering reflection"?

%RoutineAid...Support Daily Routines...Autism 
%User Engagement

%Embodying Care in Matilda...Robot...Older People in Australian Residential Care Facilities
%Efficiency, quality, and naturalness, User satisfaction survey, Predictive accuracy




\section{Disease}

\subsubsection{Dynamics of Disease in Care Work}
The stages of diagnosis that will influence the emotional coping process are dynamic and can not be solved by a single-functioning chatbot. 
Emotional needs vary significantly based on the type and stage of the disease, as well as individual and cultural factors [10]. For example, the emotional needs of a patient newly diagnosed with diabetes may differ substantially from those of someone in the advanced stages of cancer. Tailoring emotional support to the specific context of the disease and the individual patient is crucial for effective care [11].
during hospitalization, the interaction with professionals such as doctors, and nurses, before diagnosis and more stigmatized context, where the individuals explore and renegotiate their identity with themselves with available information. In the recovery process, there are occasional emotional coping needs and the need for peers to look for each other. 


%\textcite{maeng_designing_2022} state "Disability is not fundamentally a question of medicine or health, nor is it just an issue of sensitivity and compassion; rather, it is a question of politics and power(lessness), power over, and power to." %(2006: 2, as quoted in Gillies 2014 and Sleeter 2010). 

%Potential theoretical lens: X Feminist theory \cite{costello_potential_2021}
%Care: "These connections are reinforced in feminist ethics of care. In their influential essay, Fisher and Tronto suggest that “care is everything that we do to maintain, continue, and repair ‘the world’ so that we can live in it as well as possible. That world includes our bodies, ourselves, and our environment, all that we seek to interweave in a complex, life-sustaining web” [21 , p.42]. " 

"Whitehead (2012) considers the relationship between affect and feminist theory. They note that affect studies constitute an interdisciplinary space with often contradictory and oppositional takes upon the subject matter. What is clear, following Gorton (2007, 334), is that there is shared interest in the way ‘feeling is negotiated in the public sphere and experienced in the body'" \cite{goodley_feeling_2018}
%\paragraph{keywords}


% "query": { Title:(emotion AND (coping OR regulation OR support)) AND Abstract:(mental health) }
% "filter": { ACM Content: DL }

\subsection{emotion support vs regulation}
Ulman defined emotional support as the following nine be-
havior [ 81 ]: 1) preventing victims from self-blame, 2) reassuring
victims that they are not at fault, 3) understanding the incident,
4) reframing the experience, 5) not judging victims, 6) accepting
victims’ stance, 7) caring about victims’ emotion, 8) feeling sorry
for victims, and 9) empathizing with victims’ feeling. Emotional
support has been associated with improved adjustment after sex-
ual violence. Additionally, Emotional support is found to alleviate
PTSD symptoms and increase the survivors’ perceived control over
their recovery [84]. Furthermore, survivors who get emotional sup-
port have a more impressive capacity for active response to their
traumas [83 ]. Coping via emotional support may also be seen as
a sign of “resilience,” indicating the survivor’s ability to accumu-
late resources that mitigate the trauma’s effect [ 41 ]. Therefore, this
paper examines ways to provide emotional support to emotionally
vulnerable survivors to aid in their recovery from harm. This pa-
per also investigates how to ensure survivors get positive social
reactions when they first disclose their experiences."
\cite{maeng_designing_2022}


% There are many in the parent-children context for education and awareness, many in everyday life, where disease management is relatively rare. It could be a good start for a short submission. 
% Think about categorizing the emotional coping approach at the socio-technical level, interpersonal, community, and individual in the systematic review. The level of help-seeking may relate to the disease journey. 


% online data has been exploited by the tech and medical companies \cite{costello2020predictive} 

%rather than a whole intervention program, lifting the emotion can be quick. the can be ephemeral, TikTok exploited the nature of emotion and 

%We acknowledge the limitations around the word "intervention" \cite{pendse_treatment_2022}.

% Arlie Hochschild's groundbreaking work "The Managed Heart" (1983) introduced the concept of emotional labor, highlighting how certain professions, often dominated by women, require the management and display of particular emotions as part of the job [5]. This concept has been crucial in understanding the intersections of care work, gender, and emotional regulation.
% Eva Feder Kittay's "Love's Labor: Essays on Women, Equality, and Dependency" (1999) further explores the gendered nature of care work and its implications for social justice [6].
% Susan Sherwin's "No Longer Patient: Feminist Ethics and Health Care" (1992) applies care ethics to healthcare settings, challenging traditional bioethical approaches and advocating for more relational and context-sensitive approaches to medical ethics [10].

% Studies have shown that such support is associated with improved post-trauma adjustment and can play a significant role in alleviating PTSD symptoms. Moreover, emotional support has been linked to an increased sense of control over the recovery process, empowering survivors to take active steps in their healing.
% The benefits of emotional support extend beyond immediate psychological relief. Survivors who receive adequate emotional support often demonstrate greater resilience in the face of their trauma. This enhanced coping capacity manifests as a more active and engaged approach to addressing the challenges that arise in the aftermath of traumatic experiences. In this context, the ability to seek and utilize emotional support can be viewed as a sign of resilience itself, indicating the survivor's capacity to gather and leverage resources that mitigate the impact of trauma.
% Additionally, the research seeks to investigate ways to ensure that survivors receive positive social reactions when they first disclose their experiences. This initial response can be critical in shaping the survivor's willingness to seek further help and engage in the recovery process.

\subsubsection{emotion and disease information behavior}
This is despite the fact that “emotional cues” are
increasingly recognised as intrinsic to information seeking
which should also focus on people’s emotions and affective
experiences [22,44]. Emotional barriers have proved to be
significant in limiting access to health information since
emotions affect the situation, task and goal of seeking
information and vice versa [16,22]. People react emotionally
to information which impacts on understanding,
internalization, learning, and coping [44]; indeed
information processing capacity has been shown to
diminish under stress [12]. Emotions can often interfere
with clarity of thought in undertaking a task or support, or
conversely can encourage particular goals [58]. 
We have identified several needs
that arise due to the complexity and stigma associated with
HIV, including the context and emotion driving people to
seek information on HIV in the first place. This study
reiterates the particular importance of designing for real
user needs (establishing why people may be searching
online, why they may visit a site and what information they
may need to find quickly) in health information systems
where the interaction has high emotional import: many
health information resources currently do not address
people’s emotional needs and urgent goals. While our
analysis has focused on the emotional support needs linked
to technology use for HIV, \cite{smriti_emotion_2024}

\subsubsection{Computational Representation of Emotion: discrete Categorical to Dimensional}
Murray and Arnott's framework \cite{murray1993toward} classifies emotions into five categories: anger, happiness, sadness, fear, and disgust, in speech by comparing them to neutral speech based on vocal effects including Speech rate:Pitch average,Pitch range: Much wider, Intensity, Voice quality, Pitch changes, articulation. For example, anger is characterized by a slightly faster speech rate, much higher pitch, wider pitch range, higher intensity, breathy and chesty voice quality, abrupt pitch changes on stressed syllables, and tense articulation. 
\textcite{diberardino_anti-intentional_2023} highlighted a significant limitation in machine learning approaches to emotion recognition: the requirement for categorical labels. This approach constrains our understanding of emotions, which may be better comprehended through a dimensional perspective. \textcite{russell2003core} presents a compelling critique of the categorical view of emotions, arguing that it lacks a consistent methodology and scientific foundation for defining emotions. Russell points out that many scientific studies of emotion actually examine a diverse range of phenomena, including “brain
modes, actions or action tendencies, reflexes, instincts, attitudes,
cognitive structures, motives, sensations, [and] feelings” [ 62 ]. This diversity highlights the complexity of emotional experiences and the limitations of a purely categorical approach. To address these limitations, Russell proposes the core affect model as a more nuanced framework for understanding emotions. This dimensional approach maps emotional experiences along three primary axes:
Valence (positive vs. negative)
Activation (stimulated vs unstimulated)
Dominance (in control vs out of control) The model typically uses Valence and Activation as the primary dimensions, with Dominance as an optional third dimension. This framework allows for a more flexible and nuanced description of emotional experiences. He argues that it can accommodate emotional categories
without subscribing to the label as a fixed or universal ontology. It
is thus important to understand that Russel’s model of core affect
is not necessarily meant to replace the social utility of emotional
categories. \cite{lu_learning_2018, marcos_emotional_2021}.

\subsubsection{Technology Intervention: From Unimodal to Multimodal Emotion Recognition}
Human communication and emotional expression are inherently multimodal, simultaneously engaging textual, auditory, and visual channels. This complex interplay of modalities allows for a rich and nuanced conveyance of both semantic and affective information. Recognizing this multifaceted nature of human interaction, the field of emotion recognition has evolved from unimodal approaches to more sophisticated multimodal frameworks.
Traditionally, emotion recognition systems focused on single modalities, such as text analysis, facial expression recognition, or voice tone analysis. However, these unimodal approaches often fell short in capturing the full spectrum of human emotional expression. The limitations of unimodal systems became particularly apparent in ambiguous or context-dependent situations where reliance on a single channel of information could lead to misinterpretation.
The shift towards multimodal emotion recognition represents a significant advancement in the field. By integrating data from multiple sensors and modalities, these systems aim to increase the accuracy and reliability of emotional state estimates [5]. This approach mirrors the human cognitive process, where we instinctively synthesize information from various sensory inputs to form a comprehensive understanding of emotional cues. \cite{poria_review_2017} 

\section{Findings}
\subsection{Wait to see whether there is enough data}
\subsubsection{How do studies understand/define emotion?}
Emotion recognition or detection is always the first step before any interventions are made. Although several categories of emotions have been widely used in Affective Computing, there have been debates around the scientific soundness of whether there are ontological differences among these categories \cite{}
\subsubsection{Study design: Who conducts the research for whom?}
Male-centric research and theorizing:
Many of these theories were developed primarily by male researchers, often based on studies with predominantly male participants. This male-centric approach may have led to biases in how emotions are conceptualized and categorized. For instance, emotions traditionally associated with femininity (like compassion or nurturing feelings) are often underrepresented or overlooked in these models.
Western cultural bias:
Most of these theories emerged from Western, educated, industrialized, rich, and democratic (WEIRD) societies. They may not adequately represent emotional experiences across diverse cultures, particularly those with non-Western worldviews. This limitation is especially problematic when these models are applied universally without considering cultural variations in emotional expression and interpretation.

\subsection{Tools}

We grouped the tools for TMEI into five main categories: emotion tracking \& management tools, tangible devices, conversational agents, communication support tools, and virtual reality (VR). Table \ref{tab:tools-example} shows some examples of each category. It should be noted these categories are not mutually exclusive and there are cases where tools designed by the empirical studies belong to two categories. For example, studies designing robots with conversational functions were annotated as tangible devices and conversational agents \cite{10.1145/2544104, 10.1145/3421507}.

\input{tabs/jiaying-tools}
\subsubsection{Emotion Tracking \& Management Tools}
Emotion tracking tools encompass technologies designed to record and monitor emotional states, primarily serving to support emotion regulation and enhance emotional awareness through self-reflection \cite{10.1145/3628516.3655820,10.1145/3329189.3329209}. These systems employ two main methodological approaches: self-reporting and automatic detection.

Self-reporting systems require users to manually recognize, interpret, and input their emotional states as digital records. These applications are specifically designed to promote emotional awareness and facilitate self-reflection \cite{10.1145/3429360.3468190}. While these systems track and record users' emotions, they typically do not actively intervene in emotion regulation. Instead, they support self-guided emotion management \cite{10.1145/3429360.3468190,10.1145/3544548.3581048} and provide data records to facilitate communication between users and caregivers \cite{10.1145/3628516.3655820}.

To address the user burden associated with manual emotion labeling, recent research has increasingly shifted towards automated, multi-modal approaches to emotion detection \cite{10.1145/3491102.3501925,10.1145/3130943}. These systems incorporate various data sources, including facial expressions \cite{10.1145/3491102.3501925}, speech audio \cite{10.1145/3383313.3412244}, and bio-signals such as heart rate \cite{10.1145/3130943} to map synchronized emotional changes \cite{10.1145/3383313.3412244}. This automated approach enables continuous monitoring without user intervention, making it particularly beneficial for individuals facing motivational or cognitive challenges. However, studies also reported ethical risks associated with the emotion data collection \cite{10.1145/3442188.3445939,roemmich2023emotion}. 
% Meanwhile, paradigms for understanding human emotions—many of which are adopted from other disciplines by computer scientists—often assume that AI can produce an objective 'ground truth' about emotions, however, this is challenged by researchers who argue that conceptuazlizations of what emotions are different and personalized \cite{10.1145/3442188.3445939}.


\subsubsection{Tangible devices}
\label{Section:Tangible Devices}

      
% Tangible devices enhance patients' emotions by influencing their physical perceptions, naturally providing support that is well-suited and connected to their current environment and circumstances. Hence, these devices are increasingly utilized to offer in-situ support to validate and regulate emotions through sensory experiences \cite{10.1145/3491102.3502135,10.1145/3490149.3501326,10.1145/3491102.3502130,10.1145/3637409,10.1145/3569484,10.1145/3660244}. 

Tangible devices offer in-situ support to validate and regulate emotions through sensory experiences. These interventions deliver sensory feedback based on the physical and contextual signals collected from individuals, which facilitates experiential approaches to emotion regulation. Studies on artificial hugs and wearables that generate soothing sensations \cite{10.1145/3341163.3346933, 10.1145/3173574.3174069, 10.1145/3569484}  showed that technologies could mediate and simulate affective touch to provide assurance and comfort. In addition,  studies on robot companions \cite{10.1145/3434073.3444669, 10.1145/3660244, 10.1145/2544104} demonstrated the potential of embodiment to foster social interactivity and affective engagement. Relatedly, embodied toys such as interactive cushions with textile sensors and touch-sensitive plush toys embedded with speakers have been incorporated in care environments for situated support, enriching everyday life for elders and children \cite{ 10.1145/3490149.3501326, 10.1145/3491102.3502135, 10.1145/3637409}. 
\begin{figure}[h]
        \centering
        \includegraphics[width=0.75\linewidth]{figs/toyexample.png}
        \caption{Examples of Tangible Toys. From left to right: a tangible conversational agent designed for dementia patients \cite{10.1145/3490149.3501326}; an interactive cushion integrating textile sensors with touch-activated audio playback \cite{10.1145/3173574.3174069}; and a smart toy incorporating speakers and accelerometer technology \cite{10.1145/3491102.3502130}.}
        \label{fig:toyexample}
    \end{figure}
% materalize affective affordances 

% using technological sensory experiences in enhancing real-time emotional support. 
% serve as sources of emotional stability. 
% anchor 

% Embodied Toy for children  \cite{10.1145/3491102.3502135} 
% \textcite{10.1145/3491102.3502130} deployed a smart toy in family settings as an interface to elicit conversations about emotion between parents and children.
% demonstrated the effectiveness of technology-enabled objects in aiding down-regulation and promoting self-compassion during heightened emotional states. 
% "They Don't Come With a Handbook" 10.1145/3637409 Still Purrble

%
% Embodied Toy (multisensory) for PwD dementia  \cite{10.1145/3490149.3501326} 
%  Enriching Everyday Lived... \cite{ 10.1145/3316782.3321525, 10.1145/3490149.3501326}. care home residents
% a cushion equipped with conductive textile sensors that offer a touch-based input for playing audio content \cite{10.1145/3490149.3501326} 
% an interactive companion that plays sounds
% and displays colors in response to touch-based inputs and
% can mimic or react to the input of a paired device to stimulate social engagement between care home residents

% Care robots serve as companions to provide similar affordances to pets for people with dementia and depression.  

% Interactive aquarium application: touch gestures & Tangible object interaction - dementia  \cite{10.1145/3154862.3154929}

% MoodGems (Reflect)
% Assessblocks (track), 
% plasticine clay (track & express)  \cite{10.1145/3064663.3064697}
% afffective touch , slow stroking  \cite{10.1145/3569484}



% Research on tangible devcies has show npromising findings across various modalities to provide emotional care. 

% Tangible devices facilitate technology-mediated physical interactions to support real-time emotional care. Compared to other tools, tangible devices are not limited to tactile sensations; as intelligent entities, they often provide multiple forms of sensory stimulation and feedback \cite{10.1145/3569484,10.1145/3660244,10.1145/3490149.3501326}. Beyond digital interactions, they offer physical-world interaction methods.

% \subsubsection{Interactive tangible artifact}
% The environment of emotion recognition goes from the lab to a constrained field and to an uncontrolled field where multiple biological signals are collected \cite{saganowski_emotion_2023}. 
% The tangible interfaces hold promises for the embodied nature of emotions. Interacting with experiences is inseparable from bodily sensations and social contexts in comparison to studies focusing more on cognitive or behavioral aspects.


\subsubsection{Conversational agent}
\label{Section:Chatbot}
Conversational agent have shown promise in delivering therapeutic effects, with studies like \textcite{10.1145/3613904.3642761, 10.1145/3429360.3468190} demonstrating how these digital assistants can guide users to identify "thinking traps" and reframe their thought processes. Beyond directly interacting with users to provide emotional support \cite{10.1145/3479561, 10.1145/3396868.3400898}, some language-based AI systems were integrated into conversations between people \cite{10.1145/3173574.3173905}, facilitating peer-to-peer emotional communication. Similarly, the system can support users in cognitive restructuring and emotion regulation by editing their sentences\cite{10.1145/3613904.3642761}. 

% mostly via cognitive reappraisal? 

% \cite{10.1145/3613904.3642761, 10.1145/3479561, 10.1145/3173574.3173905, 10.1145/3396868.3400898}. 
 % Powered by natural language processing (NLP), AI-based systems can generate human-like responses. As a result, researchers have developed chatbots as digital emotional support agents, grounded in counseling strategies and therapeutic theories, with studies like \cite{10.1145/3613904.3642761}. 
 

\subsubsection{Communication Support Systems}
Our analysis revealed that communication support systems, primarily manifested as mobile and web applications, emerged as significant tools for enhancing interpersonal communication experiences. These systems were consistently found to facilitate emotional support and improve overall emotional well-being across the reviewed studies. The empirical research in our corpus demonstrated that emotion coping frequently occurs through peer communication and exhibits contagious properties \cite{guo2020preliminary}.
We identified three primary approaches through which these applications support communication. First, studies showed that these systems enhanced the emotional and empathetic quality of conversations through various interactive features \cite{10.1145/3442381.3450097,10.1145/3610073}. Second, researchers developed and evaluated systems that provided personalized information to support users' decision-making processes in emotional contexts \cite{10.1145/3639701.3656304}. Third, the examined applications consistently incorporated features promoting peer support and sharing mechanisms \cite{10.1145/3415183}.

%交互信息的目的， software和interactive 的优势

% Compared to VR, interactive visual media, including software and interactive video, may not offer an immersive experience but provide more convenient, real-time and continue interaction with emotion information cause they can be accessed by mobile devices.  
% This interactive emotional information enables a better content accessibility and approachability. 
% \citeauthor{10.1145/3639701.3656304} developed a narrative-based response video to help young female patients understand and navigate the fertility preservation options available to them following a cancer diagnosis\cite{10.1145/3639701.3656304}. Although it is not designed for emotion coping, it supports emotion caring.
% Similarly, some software supports users' emotions by focusing on communication rather than direct emotion regulation. 

% These applications enhance interpersonal communication experiences, thereby facilitating emotional support and improving overall emotional well-being\cite{}. For example, \citeauthor{10.1145/3130943}developed an Android app that allows users to share their heart rates via messages, providing an innovative and engaging way to express and communicate emotions. 
% Additionally, \citeauthor{10.1145/3610073} enabled partners to offer emotional support by facilitating communication about contraceptive issues. 
% Emotion tracking and recording are crucial for coping with emotions, as such software increases users' emotional awareness and reflection. Thus, some applications allow individuals to assess and interpret their own emotions.\xingyu{add example} While others rely on experts, aiming to achieve emotion regulation and education.\xingyu{add example}

% [move from Jiaying's part, feel free to add to corresponding paragraphs] Art therapy approaches facilitated by technology offer avenues for creative expression, helping users reflect on emotionally charged situations, accept negative emotions, and reframe them for resilience and self-growth. To enhance engagement and attachment, especially for specific populations like elderly individuals \cite{10.1145/2674396.2674456, 10.1145/3660244} and children \cite{10.1145/2851613.2851678, 10.1145/3491102.3502130}, gamification elements \cite{10.1145/3613904.3642123} are frequently integrated into these technological solutions.

% \subsubsection{language based tools}
% Chatbots have shown promise in delivering therapeutic effects, with studies like \textcite{10.1145/3613904.3642761, 10.1145/3429360.3468190} demonstrating how these digital assistants can guide users to identify "thinking traps" and reframe their thought processes. More immersive technologies, such as virtual reality, are being utilized to support the development of cognitive reappraisal skills, particularly among youth \cite{10.1145/3585088.3589381, 10.1145/3643834.3661570}. 

% \subsubsection{embodied / tangible tools} 
% Tangible devices enhance patients' emotions by influencing their physical perceptions, naturally providing support that is suitable and connected to their current environment and circumstances. Thus, tangible devices as a popular technology has been widely applied in emotion regulation. 

% Technologies with immersive and tactile affordances are increasingly being utilized to offer in-situ support for emotion regulation and validation, connecting real-time regulation with sensory experiences of emotions. These interventions collect sensory signals from individuals and deliver sensory feedback, facilitating experiential approaches to emotion regulation. Research has explored various technological methods to provide artificial care, with promising findings across different modalities. For instance, \textcite{10.1145/3491102.3502135} demonstrated the effectiveness of technology-enabled objects in aiding down-regulation and promoting self-compassion during heightened emotional states. Studies on artificial hugs \cite{10.1145/3341163.3346933, 10.1145/3173574.3174069} and robot touch \cite{10.1145/2544104, 10.1145/3154862.3154929, 10.1145/3569484} have shown that technology-mediated physical interactions can provide comfort and emotional support. Additionally, some studies into robot companions \cite{10.1145/3434073.3444669, 10.1145/3660244} as sources of consistent emotional stability. The affective affordances in the embodiment and interactiveness \cite{10.1145/2110363.2110398} are core for using technological sensory experiences in enhancing real-time emotional support and mental health care.

% \subsubsection{wearable devices}
% \paragraph{Tracking and Managment}
% Emotion tracking in HCI has evolved from mobile apps and wearables that rely on manual input to more sophisticated, automated detection systems. While traditional self-tracking apps offer rich pathways for reflection and emotional expression \cite{10.1145/3329189.3329209}, they can be burdensome for users, especially those facing motivational or cognitive challenges. Recent research has shifted towards automated, multimodal approaches to emotion detection \cite{10.1145/3491102.3501925}, incorporating facial expressions, speech audio, and other sensing data to map synchronized emotional changes \cite{10.1145/3383313.3412244}. For instance, EmoGlass \cite{10.1145/3491102.3501925} demonstrates an end-to-end wearable platform capable of detecting seven facial expressions using partial face images. Despite these advancements, a significant challenge remains in translating tracked data into meaningful behavior changes. Some studies address this gap by integrating emotion tracking with daily routines \cite{10.1145/3511047.3537691}, such as autism management, using visual narratives to promote sustainable habits \cite{10.1145/3544548.3581048, 10.1145/3329189.3329209}. This approach aims to embed emotional awareness seamlessly into users' life rhythms, potentially bridging the gap between data collection and practical application in emotional well-being.
% Research has underscored the importance of balancing user autonomy with optimal customization to avoid overwhelming users at the time of emotional coping; app designs need to tailor the level and type of customization to meet personalized needs of individuals \cite{zhang_designing_2021}. For example, Zhang et al. found that most users prefer lightweight tasks that align their available energy and motivation with the required effort for customization; however, users with severe symptoms benefit more from prescriptive suggestions from the app as they lack the mental capacity to mobilize change.

% \paragraph{Communication}
% Recognizing that emotion coping is often enacted through peer communication and can be contagious \cite{guo2020preliminary}, HCI scholars have integrated social mechanisms into technological designs to provide customized emotional support across various scenarios. These designs facilitate emotion tracking, expression, and negative emotion reframing among peers. For instance, the Emotion Map designed by \textcite{huang_emotion_2015} encourages users to log and annotate their emotions based on time and location, fostering emotional awareness both individually and within friend groups and communities. \textcite{10.1145/3173574.3173905} developed expressive and reflective approaches to promote mutual understanding and non-judgmental reflective listening among peers. Other research has explored leveraging peer support for personalized reframing of emotions \cite{10.1145/3479561}. Studies have also shown that receiving emotional support can sustain commitment in online health support groups \cite{wang_stay_2012}. 
% Recent studies have explored how technologies can facilitate emotional expression and support conversations about emotions between individuals, particularly within family and home settings \cite{10.1145/3628516.3655795}. 


% % \subsubsection{Interactive media for emotion expression and responses} 
% % Many studies explore the potential of using immersive and expressive media, for example, generating videos responding to emotionally sensitive responses for patients \cite{10.1145/3639701.3656304}. Virtual reality has been explored as a space for multiple purposes due to its affordances in gamifying therapeutic process and increasing user engagement \cite{10.1145/3613904.3642123}, imitating meaningful emotionally laden situations and supporting body-based experiential learning \cite{10.1145/3585088.3589381}, and create various visual representations of negative emotions through emotion regulation strategies such as externalization, seclusion, or appreciation \cite{10.1145/3643834.3661570}. \cite{shi_emog_2020} designed an interactive system that supports the sketching of emotional expressions for characters in storyboards. This tool generates character sketches with emotional expressions based on user input strokes, facilitating the creation of emotionally rich visual narratives.

% Some researchers hold that emotion perceptions and definitions are personalized. Thus, instead of intervening in the users' emotional experiences, these applications aim to co-construction of emotions with users with tracking emotions through automatic detection or self-reporting, empowering users to engage in self-reflection and management.

% \subsubsection{Chatbots and LLM}
% Conversation and dialogue-based discursive emotional coping offer a more nuanced and empowering alternative to traditional emotion regulation techniques. This approach recognizes emotions not merely as reactions to be managed, but as integral aspects of living and expressions of lived experiences. \cite{bardzell_towards_2011}. By focusing on conversational support, we can create spaces for individuals to explore and validate their emotions within the context of their personal and social realities.\cite{crenshaw_demarginalizing_1989}. AI-powered tools should be designed to recognize and address the complex interplay of factors influencing an individual's emotional landscape.

% \cite{wu_mindshift_2024}
 
% \cite{ghiotti_prototyping_2023}: Defining Design Requirements to Develop a Virtual Chat-bot for Autistic Children and Their Caregivers

% % Neglect of power dynamics:
% % Feminist scholars argue that emotions are deeply intertwined with power structures in society. Many traditional emotion theories fail to adequately address how societal power dynamics, including gender-based power differentials, shape emotional experiences and expressions. For example, how the emotion of anger is perceived and expressed can vary greatly depending on one's gender and social status.


% % Neglect of intersectionality:
% % These theories often fail to consider how various intersecting identities (such as gender, race, class, sexuality, and ability) influence emotional experiences and expressions. An intersectional feminist approach would argue for a more nuanced understanding of emotions that takes these complex intersections into account.

\subsubsection{Virtual Reality}
\label{Section:VR}
%Visual-based tools refer to technologies that provide emotion caring through visual aids or visual information. 
% Four studies designed virtual reality (VR) to facilitate the emotion coping needs of users from various backgrounds 

% including patients engaged in therapy \cite{10.1145/3613904.3642123,10.1145/3460418.3479342}, people with negative emotion \cite{10.1145/3643834.3661570}and youth \cite{10.1145/3585088.3589381}.
%Typically, such deployment was combined with various therapeutic strategies including exposure therapy ~\cite{10.1145/3460418.3479342,10.1145/3613904.3642123,10.1145/3585088.3589381}, mindfulness therapy~\cite{10.1145/3613904.3642123}, and cognitive reappraisal~\cite{10.1145/3460418.3479342,10.1145/3643834.3661570,10.1145/3585088.3589381}.

Four studies leveraged the immersive affordance of virtual reality (VR) to create vivid environments for users to express and engage with their emotions
\cite{10.1145/3613904.3642123,10.1145/3585088.3589381,10.1145/3460418.3479342,10.1145/3643834.3661570} .
% These researchers are motivated by the unique affordances of VR, particularly its ability to quickly create environments that transcend reality, for example, 
Researchers integrated various therapeutic strategies within VR including exposure therapy ~\cite{10.1145/3460418.3479342,10.1145/3613904.3642123,10.1145/3585088.3589381}, mindfulness therapy~\cite{10.1145/3613904.3642123}, and cognitive reappraisal~\cite{10.1145/3460418.3479342,10.1145/3643834.3661570,10.1145/3585088.3589381}, aimed to support emotion coping in different contexts. For instance, Soler-Dominguez et al. \cite{10.1145/3613904.3642123} built a VR garden that symbolizes users' healing journey through a variety of gamified experiences, expanding the scope of therapeutic activities in clinical settings. VR Mood Worlds \cite{10.1145/3460418.3479342} and MoodShaper \cite{10.1145/3643834.3661570} facilitated users' creative expression and reflection on emotionally charged situations, which encourages self-directed coping efforts at home. Additionally, Kitson et al. \cite{10.1145/3585088.3589381} explored VR's potential to reenact emotional scenarios that foster development of cognitive reappraisal skills among adolescents. 

% Art therapy approaches facilitated by technology offer avenues for creative expression, helping users reflect on emotionally charged situations, accept negative emotions, and reframe them for resilience and self-growth. 

% VR Mood Worlds helps emergency room patients visualize their emotions to support  \cite{10.1145/3460418.3479342}, while 
% MoodShaper allows users to manage and reflect on their negative emotions at home \cite{10.1145/3643834.3661570}. 

% ARCADIA, a VR platform used in clinical settings, enhances users' emotion regulation and self-compassion through a variety of gamified activities \cite{10.1145/3613904.3642123}. 

% Studies have leveraged VR to provide immersive experiences, which are essential for evoking emotional expression~\cite{10.1145/3643834.3661570,10.1145/3460418.3479342}. This immersive quality supports both treatments led by caregivers~\cite{10.1145/3613904.3642123} and self-care practices~\cite{10.1145/3643834.3661570,10.1145/3460418.3479342}, while also facilitating the practical development of skills~\cite{10.1145/3585088.3589381}. 

% However, studies commonly reported limitations of VR regarding equipment requirements typically limit its use to indoor environments such as clinics~\cite{10.1145/3613904.3642123}, and homes~\cite{10.1145/3643834.3661570,10.1145/3460418.3479342}. Thus, VR is primarily used for treatment rather than for tracking.
 
% These researchers are motivated by the affordances of VR regarding A, B, C. For example, one study utilized the immersive nature of VR to [unique VR features that fit the emotion coping needs of a specific population, for example, the immersive gardening for imitated but vivid experiences. multiple examples are better since we have many VR studies.] XX studies reported positive outcomes in A, B, C . XX reported non significant results. However, some qualitative results raised concerns about ...

% \subsubsection{New VR}
% A "formula" for the tool sections. Highlight, use a third-person tone, 5 studies found; 9 studies reported; The outcomes of the studies, etc. [Easieast way: You can add these to the beginning of some of your summary]
% \begin{itemize}
%     \item How many studies.
%     \item In what care context, which population, and what emotion coping.\
%     \item How the affordances of these tools match the emotion support context.
%     \item What outcomes they found regarding this type of tool for Emotion support (pros and cons)
    
% \end{itemize}

% XX studies designed virtual reality to facilitate the emotion coping needs of users from various backgrounds including children \cite{}, people with autism \cite{}... Typically, such deployment was combined with various therapeutic strategies including exposure therapy ~\cite{10.1145/3460418.3479342,10.1145/3613904.3642123,10.1145/3585088.3589381}, mindfulness therapy~\cite{10.1145/3613904.3642123}, and cognitive reappraisal~\cite{10.1145/3460418.3479342,10.1145/3643834.3661570,10.1145/3585088.3589381}. 
% These researchers are motivated by the affordances of VR regarding A, B, C. For example, one study utilized the immersive nature of VR to [unique VR features that fit the emotion coping needs of a specific population, for example, the immersive gardening for imitated but vivid experiences. multiple examples are better since we have many VR studies.] XX studies reported positive outcomes in A, B, C . XX reported non significant results. However, some qualitative results raised concerns about ...

\section{Discussion}
\subsubsection{Culture-informed coping approaches}
Rather than overwhelmingly following cognitive-reconstruction-oriented theories, researchers can explore new approaches rooted in non-Western cultures. For example, healing practices based on Indian religious traditions offer alternative perspectives on mental well-being and coping strategies. These culturally diverse approaches can enrich our understanding of mental health and provide more inclusive interventions.

\section{Discussion}
In this study, we leverage feminist perspectives on emotions to advocate for "emotion support" as an overarching goal, offering an alternative to the traditional "emotion regulation" paradigm. Through a systematic literature review of prominent HCI publication venues in the ACM Digital Library, we identified 53 empirical studies that deploy technological solutions aimed at facilitating emotional coping needs in care contexts. Our analysis reveals a rich landscape of designed tools, goals, and technological roles in emotional support work.
We uncovered a coping dichotomy in the goals of emotion regulation across the empirical studies, while also identifying additional categories of goals centered around user experience and care-centered approaches. By examining the various roles that technologies serve in care work, we have developed a nuanced understanding of the current state of technology-mediated emotion support. Building on these findings, we propose principles and design implications for a more human-centered approach to emotion support.
\subsection{Towards Human-Centered Emotion Support}
Drawing on critical reflections regarding technologies' potential for surveillance and oppression of human emotions, we propose "emotion support" as an approach that centers on humans' subjective, complex, and dynamic experiences. Feminist understandings of emotions highlight their experiential essence and enactment through social interactions. By embracing this perspective, technologies for emotional support can become more nuanced, inclusive, and effective.

\subsubsection{Beyond the Cognitive Modification Paradigm} 
% Advocate fo experiential delivery of emotion support, not just "fixing thoughts" 
Our review surfaced a cluster of interventions built on theoretical frameworks that center around modifying or taming emotions (e.g., CBT, DBT). While cognitive modification strategies and treatment-focused approaches to emotion regulation are widely used (e.g., reappraisal, reframing) \cite{kovacs1978maladaptive}, they implicitly reinforce the divide between reason and emotion ingrained in traditional Western philosophies. Feminist critics argue that such approaches can disproportionately affect women and other marginalized groups, whose emotional expressions are more likely to be labeled as "excessive" or "irrational". Researchers need to reflect on the potential harms and marginalization this paradigm may have reinforced (e.g., what is considered rational by whom in what contexts), and distinguish "non-adaptive" from "non-normative" emotional behaviors (e.g., withdrawal tendency and challenging behaviors of children with ASD at school and the elderly in residential care facilities). Interventions need to avoid displacing the individual from their physical and social environments, where norms about "appropriate" emotional expressions are fostered and inscribed. 

%  Treatments such as Cognitive Behavioral Therapy (CBT) indicate that mental representations of emotion can be linked to psychological situations. 
%  vs. cascades of emotions acted out in bedrooms...
%(CBT's Overemphasis on behavioral manifestation of emotions; less about non-adaptive, more so "non-normative"
% Researchers need to be more sensitive towards the extent to which ER goals and outcomes could be extrapolated from non-adaptive behaviors (e.g., withdrawal tendency and challenging behaviors of children with ASD at school and the elderly in residential care facilities) \cite{10.1145/3512939, 10.1145/2809915.2809917}. Such behavioral manifestation of emotions is often deemed incompatible with social expectations, and leveraged as clues to "problems" seeding intervention goals in our corpus. We caution the risks of oversimplifying emotional experiences of individuals via retrospective inferences from contextual signals. This reductionism may neglect lived experiences that manifest in ways not observable by social others without shared constellation of identities, or by the machines built on biased assumptions about emotional expressions \cite{}. 

%On the other hand, we suggest steering away from attribution of responsibility solely to "emoters" themselves as they navigate challenging emotional episodes; technologies may orient social others in the care environments, including those outside of direct care relationships, to critically reflect on how they perceive and interact with the care receivers before their emotions have been concretized. This dialectical approach weaves social agents into individuals' emotional experiences; while each interaction may seem trivial, their cumulative impact holds significance for sensitive attunement with the emoters' needs for support over time.
%may foster more sensitive attunement with the emoters' needs for support by involving social agents in their emotioanl episodes

% Section on Categorical vs. Experiential Understanding of emotions - Bridge into Design implication about experiential delivery - how do we go beyond emotion mapping problems
% Summarize the  the missed nuance in down-regulation (unintended outcomes, ambiguous emotions)  
%1) EXPERIENTIAL APPROACH: 
Challenging the dualism between mind and body, feminist theories also emphasize the embodied nature of emotions, which recognize the interconnection between physical sensations, cognitive processes, and emotional experiences.\cite{elizabeth1994volatile}. However, our analysis of employed tools shows fewer design endeavors that reflect such experiential understanding of emotions, compared to those focused on cognitive or behavioral "traces" of emotions. Beyond the problem-solving approach that silos emotions as "fixable" in thought patterns, technologies need to be more inclusive of the myriad ways emotions manifest. We advocate for more interventions that afford users the agency and rich pathways to construct their emotions as interleaved with thoughts and senses, and reflect on how sociocultural norms shape such malleable experiences.

% technologies may serve as a spring board for individuals to proactively converse with their multifacted emotional selves.

%as inseparable from bodily sensations and social contexts, 
% to flexibly modulate rather than eliminate emotional responses based on situational demands
%  involves awareness, clarity, and acceptance of emotions, 
% which are interleaved with cognition. 

% may serve as as entry points for researchers to introspect 
% CBT's over emphasis on rational thinking, overlook unconsicous process / bodily experiences, oversimplify emotional experiences and  struggles to be solvable by changing thought patterns - affordances to deeply immerse oneself in their's bodily experiences of emotions could be an alternative approach to "reframing" negative thoughts - rather, engage, converse  with the negative thoughts 
% expand upon with people’s lived experiences

%[An alternative lens from psychology] Their approach involves awareness, clarity, and acceptance of emotions, the ability to control impulses and engage in goal-directed activities in the face of negative emotions, as well as the capacity to utilize appropriate strategies to flexibly modulate rather than eliminate emotional responses based on situational demands \cite{sloan_emotion_2017}. 
% Note: this is the Gross's process model? Design implication as More Support for diff strategies rather than just "Response Modulation"?

% In addition, we advocate for empowering users to understand and navigate their rich spectra of emotions as  "bodily experiences", which are interleaved with cognition. By affording users the agency to construct their holistic emotional experiences in cognitive, affective, and physical domains, and reflect on how their emotions are malleable to sociocultural norms, technologies may serve as a spring board for individuals to proactively converse with their multifacted emotional selves.

%Further, interventions that position self-directed ER as the ultimate goal may circumvent the risk of users overly relying on technologies to learn about and engage with their emotions

%s Identity-preserving related: a spring board / canvas to explore their new identities associated with symptom development) 

%2) VALIDATION APPROACH - Neg Emo Functional, Personal Growth.
In addition, feminist perspectives often view emotions as a source of knowledge and power rather than weakness \cite{barrett2006emotions}. This viewpoint encourages validation of emotional experiences and recognizes their importance in decision-making and social change. However, our review uncovered a predominant down-regulation goal, which silenced the generative roles of negative emotions (e.g., anxiety and anger may sharpen focus and fuel motivation but are often presumed to impair well-being and hinder the enactment of rational decisions). More interventions are needed to help users understand, validate, and learn from their emotional experiences, rather than suppress or control emotions as the nemesis of rationality. This validation-driven approach can also de-escalate intense affect if individuals themselves deem it necessary, without compromising the integrity of their rich emotional life and their opportunities to avail affective signals in decision making. 

\paragraph{Design Implications: }
Researchers may adapt the cognitive modification paradigm as a departure point to critically probe how lived experiences of individuals align with and/or diverge from these coping strategies. Given the potential risks of this paradigm in divorcing one's emotions from bodily sensations, this approach holds particular importance for populations that struggle with interoception, which restrains their ability to access and interpret somatic signals to label their thoughts and feelings. 
% Such reflexivity may also unveil distinct sociocultural norms cast onto the local practices of emotion coping and desired support. These insights on the roles of emotions in social functioning across different populations can inform community-based intiatives that address...

\xingyu{Relatedly, enhanced engagement with a diverse range of biodata while acknowledging the plurality of human bodies can foster shared living and knowing and alternatives forms of care~\cite{10.1145/3532106.3533477, 10.1145/3130943}. Recognizing the limitations of categorically labeling emotions, we highlight the intricate balance between ambiguity and clarity to  facilitate embodied interaction with the feelings of oneself and others \cite{costanza-chock_design_2020, 10.1145/1094562.1094570}. This approach not only centers users to flexibly interpret their bodily signals, but also offer them a sense of comfort and agency with technologies tapping into their intimate space \cite{grill_attitudes_2022}. For instance, \citeauthor{10.1145/2901790.2901850} show how the ambiguous clothing-based displays of skin conductance validate one's feelings and offer social cues to others; such interfaces enable users and those around them to collaboratively interpret and create meanings for their emotional signals}.
% leave room for affective sense-making.
% Their design incorporates "design-as-affect," allowing people to use skin conductance displays to facilitate social performances.
%Grill & Andalibi - mentioend ambiguity as comforting as it preserves agency, pitfalls of algorithms being too accruate; less about advancing emotions as embodied?  c

Designs may also strive to preserve the agency and breathing space of individuals to process intense, negative emotions, which may be challenging in the moment but instrumental for personal growth and long-term well-being. While we acknowledge VR's potential to support body-based experiential learning, which leverage immersive affordances to facilitate reenactment of emotionally laden situations \cite{10.1145/3585088.3589381, 10.1145/3613904.3642123}, we invite design provocations that embed more accessible, familiar materials into everyday environments to craft sensory narratives of negative emotions; this approach may mitigate the harm of overwhelming emoters with heightened salience of negative feelings. To this end, our work echoes the feminist commitment to shifting the goals of sociotechnical systems from "managing" to "nurturing" people \cite{bardzell_towards_2011}; the journey of negative emotions can be uplifting if guided with sensitive technology designs, ensuring that user autonomy is interwoven within interventions.

% imitate meaningful, emotionally laden situations and support body-based experiential learning , and create various visual representations of negative emotions via externalization, seclusion, or appreciation \cite{10.1145/3643834.3661570}.  emotionally rich narratives
% invite design provocations for translating VR's potential for body-based experiential learning into everyday care environment, incorporate art therapy approaches work with mundane materials in daily life - 
% loss of control 



% % \subsubsection{Interactive media for emotion expression and responses} 
% % Many studies explore the potential of using immersive and expressive media, for example, generating videos responding to emotionally sensitive responses for patients \cite{10.1145/3639701.3656304}. Virtual reality has been explored as a space for multiple purposes due to its affordances in gamifying therapeutic process and increasing user engagement \cite{10.1145/3613904.3642123}, imitating meaningful, emotionally laden situations and supporting body-based experiential learning \cite{10.1145/3585088.3589381}, and create various visual representations of negative emotions through emotion regulation strategies such as externalization, seclusion, or appreciation \cite{10.1145/3643834.3661570}. \cite{shi_emog_2020} designed an interactive system that supports the sketching of emotional expressions for characters in storyboards. This tool generates character sketches with emotional expressions based on user input strokes, facilitating the creation of emotionally rich visual narratives.

% HOPE via Tangible -> Embodied Nature of Emotions (Interactive tangible artifact)
% The environment of emotion recognition goes from the lab to a constrained field and to an uncontrolled field where multiple biological signals are collected \cite{saganowski_emotion_2023}. 
% The tangible interfaces hold promises for forgrounding such embodied nature of emotions. Interacting with experiences is inseparable from bodily sensations and social contexts. 


\subsubsection{Acknowledge the diverse needs of emotion support}
%\subsubsection{Broaden the scope of "desirable" emotions}
%(Note: This section expands on how to Move Beyond Up-regulate + Down-regulate)

%1) Beyond modifying "thoughts" - healthy engagement with negative thoughts (challenge "rational thinking")
%(Embrace the potential of negative emotions to foster personal growth. )

%moved from intro: 
%For instance,  Bennet and Rosner \cite{bennett2019promise} surfaced the pitfalls of researchers' "empathy activities" in displacing users from their lived experiences; accordingly, they proposed "being with" rather than "being like" the intended users throughout the design process. In the realm of affective health, 
%For example, Williams et al. identified how disabled users were burdened by the expectation of "positive" changes imposed by technologies. the delineated a "counterventional" approach that foregrounds .
We unveiled a focus on interlacing sociability with positivity in the up-regulation coping dichotomy, which reflects the constant push for feeling joyful and energetic inherent in extant design solutions. This approach may inadvertently strain how individuals attend to and explore the array of their emotions as they naturally arise, especially for populations prone to volatile emotional changes due to health complications. In other words, inertia is not always an indicator for "unwell" - the stance on "activating"  individuals with interactive, sensory-rich stimuli signals lack of respect and care for individuals' private space, wherein they process feelings or enjoy solitude when they themselves deem appropriate. Researchers and designers need to gauge the contextual preferences of individuals, regarding their unique emotional needs and varied capacities to engage in interventions (e.g., whether, when, and how they want to be stimulated and nudged for social interaction).
%2) Beyond modifying "maladaptive" emotional behaviors 
%“So [I’m] being assessed for my behaviour, not for what I’m feeling. Not for my story. They’re not interested in that.”—Stolen Generations survivor Aunty Lorraine Peeters"
% How do we give the "stories" back to users that are abstracted as metrics - co-design but via altnerative "languages" of care receivers (e.g., tangible materials) 

Our review also shows that the process and outcomes of down-regulation were more complex than mere comparisons of emotional states measured in-situ (e.g., self-report misaligned with physiological measures, unintended outcomes of negativity focus). In addition, the majority of studies in our corpus framed UX goals in terms of serving ER goals, which positioned low usability and user satisfaction as barriers to realizing the potential of design solutions in emotion support. However, we caution extrapolating too far from quantitative UX metrics, as promising results on user engagement with the device or system per se do not equate to clinical effectiveness (e.g., affective responses towards social robots did not translate into therapeutic effects \cite{10.1145/3434073.3444669}), nor do they account for emotional changes when technologies take on the roles of generators, mediators, or nudges in people's emotional experiences. 

While we highlight the studies that uncovered unique design challenges within qualitative feedback \cite{10.1145/3415183}, we acknowledge the feminist principle of agnosticism about quantitative and qualitative methods, which both bear risks for unjust representation of the people \cite{bardzell_towards_2011}. Thus, we advocate for triangulating assessment of user engagement and broader user experience via self-report measures, interviews, field observations and/or behavioral analyses to enrich understanding of individuals' emotional experiences.  
% give rise to the match or mismatch between expectation and performance

\paragraph{Design Implications: }
We advocate for empowering the "people" that we aim to extend care towards to co-construct the goals and approaches of designing technology-mediated emotion support \cite{bardzell_towards_2011}. While co-design workshops may garner rich insights on what feeling "better" entails for different user groups, we highlight the need for alternative, sensitive methods to engage individuals, who may experience challenges in communicating their preferences due to health conditions. Inspired by the approach of "making as expression" in art therapy\cite{}, we suggest researchers draw on materials beyond verbal modality as authentic languages of care receivers to facilitate fluid expression of their identities and emotional needs.

% From Being "LIKE" to Being "WITH"
% Commitment 1: Rather than seek to represent another’s experience, we seek partnerships in imagining the design encounter.
% Commitment 2: Rather than achieve an understanding, we seek a process of ongoing attunement.
% Commitment 3: Rather than attempt symmetry, we recognize and work with asymmetry.
% codesign: "building consensus, or understanding each other's perspectives, can improve the human-centeredness of mental health AI research" \cite{yoo_missed_2024}. 

%CITE "MAKING AS EXPRESSION" - ART THERAPY PRACTICES; CITE PROMISE OF EMPATHY 3 COMMITMENTS
% "materials as language" in art therapies to inform.....sensitive towards what materials to  bring into co-design session as they signal expectations to participants...
% cite clay paper

Relatedly, we urge for critical reflection on whose voices to account for throughout intervention development. Beyond cultural, societal norms of how emotions "should" be expressed,  researchers need to proactively learn about and stay informed of how intersecting identities shape individuals' emotional experiences and their distinct needs for emotion support \cite{10.1145/3078072.3079742}. The vast data sources in the digital space (e.g., online communities) present opportunities to learn from authentic narratives of diverse populations and local practices of marginalized individuals, whose voices tend to be drowned out by power differentials \cite{pendse_treatment_2022}. 
% CITE Pendse et al., 2022 GROUP SYMPTOMS VIA GROUND-UP APPROACH AS BASEMENT MEASURES 

% Building on the "experiential delivery", here contrast the multi-sensory approach, highlight how NON-verbal cues or SELECTIVE usage of sensory stimulation / affordances might be favorable to populations with limited capacity for engagement (avoid sensory overload, back to the agency theme, choose which modality to engage with) 

%[Echo Social Construction of Emotions - Intersectionality]
% e.g., children acting out in school due to lack of awareness and understanding of their emotional experiences, but their behaviors were treated as "abnormal" and considered a target outcome to be modified in ER interventions...

% \paragraph{Design Implications: } Previosu UX Implications
% need explanation
% Researchers need to attend to contextual signals in care environments and gather user feedback over the course of design deployment. 
To account for the temporal dynamics of emotions while users journey through their disease management, researchers could map different sources of quantitative and qualitative insights over the course of intervention. This approach may help identify the design components that overlook users' emotional needs, which precipitate dissatisfaction and disengagement. For instance,  user satisfaction metrics can signal overall attitudes and alignment with user expectation; when paired with qualitative feedback, they may reveal reasons behind such user sentiment and when such "estrangement" with technologies occur. As users' cognitive and affective needs evolve along with their symptoms, technology designs need to keenly adapt to how users orient themselves to care. 
% In doing so, interventions can more sensitively support the dynamics of disease management by considering the shifting roles of technologies in users' care journey. 


% In particular, users might be more engaged in intervention when their contextual needs are met, and become disengaged or fall out of touch with the intervention device when their needs have shifted. 

% Very few studies evaluated "usability" from perspectives of Diff Stakeholders or Proxy Eval by caregivers...we advocate for juxtaposing usability issues pointed out by / or ER outcome evaluations by caregivers, providers, individuals in needs and see where the misalignment occur...
% Proxy: e.g., schools/institutions but not the receivers 
% (pros vs. cons, reality constraints/ feasibility in gaining user feedback from the affected population)...
% Other stakeholders: e.g., 1 study drew on expert reviews...; ToMtool: ease of use evaluated by 1 senior + 1 therapist, NOT child)...

% e.g., cognitive and physical burdens in using intervention device given their unique care contexts/journeys 
%- observations of cognitive + affective engagement with devices/systems
%- observations of perceived immersiveness / realism and naturalness  


\subsection{Situating roles of technologies within the socio-tech ecosystem}
We identified various roles that technologies serve in supporting people's emotions in the carework context. This section outlines several key implications. 

\subsubsection{Design for Caregivers: Human Care and Gendered Work}
Our review reveals a significant trend in using sophisticated computational methods to generate algorithm-driven artificial care as an alternative to human care, particularly when the latter is unavailable or burdensome. However, this approach overlooks crucial feminist perspectives on care, which emphasize that emotional needs require spaces, time, and interactions that cannot be easily replicated by machine-generated "emotional expressions" devoid of genuine human experiences. Recent studies have shown that vague or irrelevant digital empathy provided by chatbots and LLMs can be superficial, potentially causing emotional harm to users rather than providing authentic support. Our review also uncovered how embodied agents may blur the lines of artificial care for elders and children, bounding their involvement and emotional rhythms with these agents \cite{10.1145/3173574.3174069, 10.1145/2110363.2110398}. Recognizing that emotions are interwoven in human interactions and cannot be simply addressed by digital surrogates, designers should reconsider approaches that aim to replace human care with artificial care. 

Further, a notable gap emerged form our corpus in addressing the gendered labor reality of emotional support. Feminist scholars recognize emotional support as a form of labor crucial to fostering engagement and relationships \citep{hochschild2019managed,smriti_emotion_2024}; emotional labor is deeply embedded within physical interactions with care receivers and institutions. By highlighting the often invisible nature of emotional care, feminist scholars challenge societal norms that expect women to naturally provide this care without recognition or compensation. Building on this perspective, we underscore how care provision encompasses organizational, physical, and emotional labor, which presents challenges and opportunities to design technologies for sustainable caregiving. 

On one hand, by easing physical demands, technologies can allow caregivers to focus more on meaningful interactions that forge trust with care receivers \cite{llubes-arria_emotional_2022}. On the other hand, we highlight the potential of emotion tracking and communication support systems to contest and reframe the gendered narratives of "empathy" (e.g., who can, and are assumed to be good at empathizing in care relationships). The potential barriers to understanding emotional needs of care receivers are not bound by caregivers' gender identities, rather, by their own lived experiences that render perspective-taking more or less challenging. Thus, we call for more interventions that shift the discourse of empathy from being a gendered "trait" to a commitment willing to be made, which can be easier to fulfill via attunement in care work supported by technologies. In this vein, technologies may soften the normative, gendered boundaries of who ought to deliver emotion support, zooming out on the intrinsic value of human care. 
% reducing the asymmetries of data around emotions of care receivers, 
% as well as addressing the informational needs of caregivers as they navigate treatment procedures and seek institutional assistance. 
% However, technologies may fill this gap by reducing asymmetries of data around individuals' emotions, 
% infnormational support - tech foregorunds the "data" about the emotions of the care receivers , acknolwedge the ' emotional struggles of caregivers as they interface with these emotional data (how to present these data in a way that highlights "opportunities for foster bond"
% Cite studies informal caregivers mention the emotional burdens of logging children's challenging behaviors, during reflection
% CITE MyCalendar, GeniAuti

\paragraph{Design Implications:}
While algorithm-generated empathy and cognitive reappraisals have their place, embedding them within a human-moderated framework is essential. This approach not only preserves the human-to-human connection vital to emotional support but also addresses pragmatic concerns, ensuring that unpredictable situations and emerging malfunctions – particularly common in care contexts where extreme and sensitive emotions frequently arise – can be handled appropriately.  Relatedly, we highlight the potential of using linguistic intelligence to connect people, facilitating support through algorithm-mediated communication (e.g., refer to others' stories and experiences, provide direct and navigational help).

Researchers and designers must adhere to the "do no harm" principle and ensure technologies don't solidify or expand power asymmetries (e.g., design decisions that restrict human modulation of care, restrict informal caregivers' access to gaining support in their care work). It is crucial to maintain flexibility and creativity that foster and enrich modes of care delivery; for instance, beyond mere shortcuts to correct or fix care receivers' emotional responses, designs can embed caregivers earlier in their emotional journey  \cite{10.1145/3490149.3501326,positech}. We highlight studies that empower emoters to express and log their feelings via nonverbal means, which can also encourage caregivers to engage with tracked data that update their experiential understanding of care receivers' emotional needs \cite{10.1145/3152771.3152793, 10.1145/3512939,10.1145/3628516.3655795}. As only human caregivers can reflect on and interpret these tracked data meaningfully, by drawing on their own lived experiences and unique interactions wtih the emoters from other care contexts, this collaborative approach to reflection can also re-center the human in care work. Through these integrations that acknowledge the irreplaceable value of human connection in emotional support, technologies may complement and enhance human care rather than attempting to replace it.
% overcome the barriers of gendered care work 
% by encouraing reflections on part of caregivers...to depict the care receivers' emotional landscape.
% also roundabout way to ensure" human invovlvement" in care delivery - 



% affordances for caregivers to document their emotions alongside care receivers...are there studies already in a similar vein?

% Providing care for mentally ill people places the caregivers at the intersectional vulnerability with the attached stigmas, non-paid emotional labor, and. High tech solutions may broaden the gap between classes and detorite the injustice in care access. The current technological and digital design is leading the research away from the origin connections between people, emphasizing the "independent" capabilities of technologies in circumventing the structural, organizational, cultural, and social barriers. However, care is intrinsic pulse that is written in human nature that the informal caregivers, the family are willing to sacrifice part of their autonomy. The true care can not be replaced by the artificial emotions and the value of such voluntary actions should not be colonized by the market perspective. Turning to the AI-mediated caring chatbot is a turning away and escape from the 

%\xingyu{Instead of directly intervening in people's emotional experiences, they aim to enhance emotional expression, awareness, and communication through various interfaces—including tangible interfaces, online applications, and VR—to address power imbalances in emotional communication. For instance, \citeauthor{10.1145/3610073} designed an application prototype to facilitate communication between users and their partners, supporting them in engaging more fully and expressing emotional support. 
% Although some studies aim to strengthen communication between specific groups and their caregivers\cite{}, when the focus is therapeutic, the emphasis often shifts toward emotion regulation and treatment. Therefore, we recommend that future designs consider the care recipients' control over the intervention and their comfort in expressing themselves.}



\subsubsection{Design for Care-Receiver: Identity Preservation Across Care-Seeking Journey}
While many studies in our corpus focus on general wellbeing contexts \cite{sanches_hci_2019}, we highlight research that addresses emotion support for individuals with diseases, who often experience intersected marginality complicating their emotional experiences throughout the disease management journey. Rather than aiming to "regulate" emotions, these studies emphasize care-centered goals of facilitating non-judgmental validation and identity construction.

Identity plays a pivotal role in how individuals experience and cope with illness, influencing their symptom recognition, disease interpretation, self-reflection, and help-seeking behaviors \cite{pelttari_emotional_2022}. This complex interplay manifests in varied psychological states and emotional needs throughout the disease journey. Patients often grapple with anxiety, depression, and fear, compounded by feelings of uncertainty and loss of control. As evident in our corpus, broken routines intensified the anxiety of individuals with autism; everyday barriers to sensorily engage with the world destabilized elders' sense of self  \cite{10.1145/3544548.3581048, 10.1145/3490149.3501326}); a whirlwind of emotions arose from societal expectations inscribed onto the pre-illness identities of young female patients, as they navigated decisions on cancer treatment and fertility preservation \cite{10.1145/3639701.3656304}; inpatients struggled to live with their volatile emotions when forced to familiarize oneself with different forms of care related to treatment procedures \cite{10.1145/3415183, 10.1145/3109761.3109790}. 

% emotional  rhythms of individuals fluctuate across their daily activities
% treatment procedures also imposed challenges for 
% as young female patients navigate fertility preservation decisions upon cancer diagnosis, 
% ADD Examples from findings, how emotions change thorughout disease management, 
% --> 3 types of  change arranged in "scope": within 24 hours - daily routine < during medical decision amking < across symptom development / treatment procedures) 

% ADD "Limited control over one's enviornemnt" - What types of environment? Residential care, inpatients (loneliness, isolation given treatment) 
% or treatment procedures inhibits "inpatients" from fully engaging in intervention? 

Recognizing such complex identity perceptions in healthcare contexts, our review underscores the need for personalized, identity-sensitive support in health technology design. In cases of severe or life-limiting illnesses, traditional emotion regulation strategies like problem-solving may prove inadequate or counterproductive \cite{goodley_feeling_2018}, particularly when situation modification is not feasible due to limited control over one's environment \cite{smith_digital_2022}. In addition, our analysis of the extant tools revealed the need for designers to recognize the power dynamics that different technologies impose, regarding when and how individuals interact with their emotional selves. For instance, the device constraints of VR and wearables often imply that users are compelled to stay engaged in interventions. In contrast, self-reported software and communication support systems offer users greater autonomy to choose their level and mode of involvement. Technologies should adapt to users' varying energy levels and motivation, which fluctuate with symptom severity and the contexts in which emotions are experienced and expressed  \cite{zhang_designing_2021}.  
%  provide tailored support that preserves user autonomy. 
% in controlled environments, abstracting them from real-life scenarios where emotions are experienced and expressed


% Ref studies on embed design solutions into care environments & mediator of power dynamics, recognize home as home - how do tech gauge " varying energy levels and motivaiont? by tunning into daily routines (privacy concerns) 

% PRE-ILLNESSS IDENTITY: The need to maintain a sense of identity and self-worth is also paramount. Charmaz (1983) describes how chronic illness can lead to a "loss of self," where individuals struggle to maintain their pre-illness identity [6]. Interventions that help patients find meaning in their experiences and maintain or adapt their sense of self can be crucial for emotional well-being [7]. 
% ISOLATION / LACK OF SOCIAL CONNECTION: Furthermore, the emotional needs of patients often extend to their relationships and social interactions. Diseases can strain relationships and lead to feelings of isolation or burden [8]. Supporting patients in maintaining and nurturing their social connections is essential for their emotional health. 

\paragraph{Design Implications:}
Designers should incorporate features that allow users to document and reflect on their pre-illness identities and evolving self-perceptions, such as digital journals or interactive timelines. Narrative-based coping strategies can be integrated to promote meaning-making and reconstruct identities. Implementing gradual goal-setting frameworks that align with users' evolving capabilities can also support identity preservation. Thus, we highlight interventions infused within the ebbs and flows across individuals' daily routines and symptom development. In so doing, technologies may address the emotional challenges rooted in lived experiences, sparking sustainable behavior changes that align with people's new identities \cite{10.1145/3544548.3581048, 10.1145/3628516.3655795}. It is vital to ensure cultural competence in these designs, acknowledging how diverse backgrounds influence identity and illness experiences. Interventions also need to account for individual differences beyond classification within the same health condition. 
% learning about who they were before

In addition, flexible communication tools may help users maintain social connections while validating the temporal dynamics of identity shifts and emotional needs. For instance, by orienting users to people with shared facets of identities or in a similar stage of disease management, technologies may help individuals embrace the fluid nature of their self-concept as they co-construct identities with social others navigating care\cite{10.1145/1517744.1517804}. Through both inter- and intra-personal approaches, technologies can better support users in maintaining or adapting their sense of self throughout their care-seeking journey, which fosters resilience and holistic emotional health.

% Add in our corpous, one study mention ppl look for others NOT with the same symtom / diagnosis, but similar emotional experiences, or who are also going through emotional roller-coaster as a way to "validate" their own experiences (informational vs. experiential validation)

Lastly, designs need to avoid compromising individuals' sense of ownership over their emotions, especially when technologies tap into their personal space in the name of emotion support. We acknowledge the challenge to accurately capture and represent emotional experiences via contextual signals, while embedding consent-forward yet feasible mechanisms to gather user feedback in care provision. This barrier could be particularly salient for populations who are disconnected from their own bodies due to health complications. Hence, we foreground the need for ethical data use for personalization while striving for contextual sensitivity. Recognizing algorithmic accountability and emotions as a source of sensitive data \cite{andalibi_human_2020}, interventions should aim to provide tailored support that preserves user autonomy.


% maybe urge for proxy consent and ongoing attunement with such shfited needs via caregivers of those who struggle to verbalize / express their preferences? Advance directive consent?  "Advance directives are utilized when an individual cannot provide informed \textit{consent} or refuse due to incapacity."
% Connect "ethical data use for personalizaiton" with cluster of studies on need for contextual signals, embed intervention into daily routines 
% Dillemma in getting closer to "ground truths" of emotiosn; in order to accurately represent indvididuals' emotional experiences (represent one's emotional self, identity preserving), pervasive sensing seems inevitable, which ironically compromises one's freedom to choose whether and how to share data around their emotions
% -> design provocations for feedback mechanism, too much self-report too burdensome, bio-signals do provide valuable passive signals that one cannot consciously recall, especially for populations who feel disconnected from their bodies. 


\subsubsection{Design for Relationships: Power Dynamics in Carework}
\cite{crenshaw2013mapping} recognizes that emotional experiences are influenced by various intersecting identities such as gender, race, class, and sexuality. The intersection of emotional support, caregiving, and technology raises important questions about the nature of care and the potential impacts of technological interventions. While technology may offer solutions to some aspects of caregiving, it is essential to consider how it might affect the intricate balance of emotional labor and connection that characterizes human-to-human care relationships. \textcite{smriti_bringing_2023} highlighted that caregivers often hold a strong aversion towards certain emotion-intense tasks. Paradoxically, while the logistical aspects of care work are less addressed in research, more studies are attempting to replace the emotion-intense interactions that caregivers actually value \cite{schorch_designing_2016, smriti_emotion_2024}. This disconnect underscores the importance of user-centered design in affective health technologies.
%The loci of assessment may be expanded to different stakeholders. By juxtaposing usability issues or ER outcomes evaluated by providers and recipients of care as well as institutional representatives, researchers may identify the misalignment on how emotions are experienced, expressed, and perceived by individuals with distinct roles in care relationships. The breadth of perspectives may also pinpoint the design constraints unique to each care context and disease journey.

In addition, the loci of assessment may be expanded to different stakeholders. By juxtaposing usability issues or outcomes of emotion support evaluated by providers and receivers of care as well as institutional representatives, researchers may identify the misalignment on how emotions are experienced, expressed, and perceived by individuals with distinct roles in care relationships. The breadth of perspectives may also pinpoint the design constraints unique to each care context and disease journey. 

\paragraph{Design Implications:}
Future work in this field should strive to balance technological innovation with a deep understanding of human emotional needs and preferences. Designs should acknowledge that "feelings are negotiated in public sphere" \cite{gorton2007theorizing} and consider the ripple effects of one's emotions on others involved in the care relationship. Communication support systems could help address unintentional disconnects between caregivers' good intentions and their delivery of care at inopportune times.
% Some caregivers would like to learn about how dementia develops in order to anticipate changes, prefer receiving info in person rather than via "a computer" 
% infnormational asymmetries also relate to power imbalance? who is it to say what forms of care to deliver / receive?  - insufficient info, rely on others to navigate one's emotional turbulance
%Houben et al., 2024. Design Opportunities for Care Transitions in Dementia: Understanding Informal Caregivers’ Experiences Through a Practice-Informed Approach CHI 2024
% Prior research has shown that non-verbal cues hold promise for reducing friction in care work, especially for populations with reluctance for directive care

Collaborative and ecological perspectives emphasize that support from interpersonal relationships and community are strong motivators for seeking professional help \cite{migliorini_help-seeking_2023}. Integrating these perspectives could lead to multi-level intervention programs that not only increase individuals' knowledge about mental health symptoms and coping strategies but also facilitate the formation of supportive peer networks that foster sustained help-seeking behaviors \cite{kaziunas_precarious_2019, murnane_personal_2018}. These designs should aim to balance power dynamics in carework, recognizing the complex interplay of emotions, responsibilities, and relationships within the care ecosystem.


\section{findings}
\subsection{Roles in Care Work}
Viewing technology-supported emotion coping through a feminist lens as care production, we explore technology's roles in this process. We identified three roles the tools for technology-supported emotion coping played including generating artificial care, nudging behavior changes, and mediating power dynamics.  

\subsubsection{As a generator of artificial care}
Artificial care refers to non-human-generated emotional support, such as simulated hugs and empathetic responses from machines and algorithms. This approach addresses the labor-intensive nature of providing emotional support, as noted in studies on the costly process of constant comforting in caregiving.
Our corpus reveals a significant focus on tools generating artificial support. Virtual Reality (VR) \cite{10.1145/3643834.3661570, 10.1145/3563657.3595998, 10.1145/3491102.3517492, 10.1145/3357236.3395560} and tangible devices \cite{10.1145/3410530.3414375, 10.1145/3173574.3174069, 10.1145/3491102.3502135} are commonly used to create rich sensory interactions eliciting emotional responses. Chatbots \cite{10.1145/3589959} provide artificial care through conversational interfaces, offering readily available empathetic responses.
These artificial care systems show the potential in alleviating caregivers' emotional labor burden by providing constant, tireless simulated support. However, studies report limitations and drawbacks, including challenges in adapting to nuanced contexts, risks of unrealistic attachments, and concerns about the authenticity of machine-generated empathy.

Recognizing these complexities, researchers have explored integrating artificial care within human-mediated processes. For example, studies on AI-assisted suicide detection and emotional support systems for online counselors \cite{10.1145/3613904.3641922} aim to enhance human capabilities in providing responsive and empathetic care.

%robots both tangible and narratives for artificial care. 
%Kitson et al. 2024 mentioend "on-the-spot experiential-based interventions" 

%emotions as individual, internal experiences, neglecting the social and relational aspects of emotions that feminist theorists often emphasize. This individualistic approach may undervalue the importance of collective emotions and emotional experiences shaped by social identities and relationships.



\subsubsection{As a mediator to intervene in power dynamics}
%tangible device as an interface such as robots that facilitate one-on-one among elder adults.
Technology in caregiving contexts is increasingly being leveraged to address and potentially rebalance inherent power dynamics, which often lead to the suppression of feelings and experiences, particularly for those in vulnerable positions. This mediating role of technology aims to empower individuals and create more equitable emotional landscapes within care relationships.
At the core of this approach is the recognition that emotional coping needs frequently stem from power imbalances in real-life situations. Technology interventions are being designed to subtly or explicitly modify these dynamics, offering new channels for expression and support. For instance, \textcite{10.1145/3610073} focused on romantic relationships, where contraception responsibility often falls disproportionately on one partner, technology has been used to initiate conversations about birth control, aiming to increase couples' accountability and create opportunities for mutual emotional support.
In parent-child relationships, where children may have limited emotional expression abilities, researchers have explored innovative solutions. \textcite{theofanopoulou_exploring_2022} investigated the use of embodied, in-situ toys as novel channels for children to express their experiences and emotions to parents. This approach seeks to amplify children's voices in the caregiving dynamic, potentially equalizing the emotional exchange between parent and child.

Similarly, in professional care settings, efforts are being made to enhance the visibility and agency of care recipients. Studies have focused on designing tools to improve caregivers' emotional recognition skills \cite{10.1145/3575879.3575997} and provide support \cite{10.1145/3415222}, indirectly empowering care recipients by ensuring their emotional needs are better understood and addressed. 
Some studies challenge medicalized views of technology in care settings. The emphasis on recognizing care homes as 'homes' rather than clinical environments for people with dementia \cite{10.1145/3490149.3501326} represents a fundamental reframing of power dynamics. This approach seeks to prioritize the autonomy and dignity of residents, using technology to create more homelike, less institutionalized environments that respect individual agency. These approaches recognize that emotional well-being is intrinsically linked to issues of agency, visibility, and mutual understanding.


\subsubsection{As a nudge for action/behavior change}
%gamified
%nudges through social awareness

%(Differentiate studies that\textbf{ do (not) }go beyond "EmoAware" stage to \textbf{scaffold} ER)
%  Aware (Early Stage): Claimed to promote emotion awareness, mindfulness, and reflection
%  Skill (Later Stage) : 
In caregiving contexts where physical demands often overshadow emotional needs, technology is emerging as a crucial tool to highlight and maintain the visibility of emotions. Studies explore ways to uses tangible devices and self-tracking apps to help users identify and label their affective states in relation to daily experiences \cite{10.1145/3491102.3501925, 10.1145/3429360.3468190, 10.1145/3152771.3152793, 10.1145/3643834.3661570, 10.1145/3628516.3655795}, serving as persistent reminders for emotional awareness amidst intensive physical care tasks. Other research has focused on visualizing emotions for autistic individuals to aid in interpreting emotional cues from others \cite{zolyomi_emotion_2024}, and on utilizing caregiver-tracked data to inform clinical recommendations for managing challenging behaviors in children \cite{10.1145/3512939}.

This proactive stance aims to intervene earlier in the emotion regulation (ER) process, moving beyond immediate emotional state modification to foster long-term awareness and skills. These interventions seek to help individuals develop more adaptive ER strategies over time; however, empirical evaluation of these approaches remains limited. Only a few studies have employed established measures like the Difficulties in Emotion Regulation Scale \cite{10.1145/3643834.3661570}, assessed changes in beliefs about emotional controllability \cite{10.1145/3491102.3502130}, or explored perceived learnability of ER skills post-intervention \cite{10.1145/3613904.3642761}. Qualitative insights from user evaluations suggest these designs may indeed promote reflection and heighten awareness of emotions and negative thought patterns \cite{10.1145/3628516.3655795, 10.1145/3479561, 10.1145/3491102.3501925}, pointing to their potential for improving emotional well-being and interpersonal functioning within caregiving relationships.

% Our results illustrate that, so far, our users do not use online social networks, and even their real-world social connections are decreasing due to limited time, energy and options. Building a dedicated community for informal caregivers has been our ambition since the foundation of the project. Yet, with more understanding of  the field, we are ever more aware of the need for social support for this population (e.g. experience on fighting stigmatization and shame, psychological counseling, social inclusion, online/offline events, and care for one’s own situation). Considering the lower-than-average physical mobility of this user group, especially in rural areas where offers are even more limited, the platform might also provide mobility support (e.g. public connection, taxi, car sharing [45]).

% People seek emotional validation that their feelings are valid,  "A state of emotional validation is salient when one believes that an “activity, emotion, belief, sense, or other experience or response” is “relevant and meaningful” While seeking a sense of perceived normalcy was a subjective experience, we identified informational and experiential validation as two related themes describing the participants’ shared experiences and journeys toward achieving emotional validation. "\cite{andalibi_sensemaking_2021} The validation can be only achieved through discourses, conversations, and narratives in verbal or written languages. People may go through the reflection through a personal diary or with others. 


==> Anotes.tex <==
Meeting Agenda
Greetings
Introduction: Intention to gather people
A brief report on the summary of revisions
The current version



Working In progress
Clarify and concise the Introduction
Enhance the logics and storytelling of Related Work

Minor
Adding Desmond as a potential author
Addressing other minor suggestions, adding literature,
Writing Summary of Revisions
Updating the Table 2, replacing tools with approaches

Requests:
(section 2, findings 5.1 and discussion)


Things to do:
Before Monday

Sec 3 logic
Method logic

Discussion revision

Polish and citations
Method table

My findings revision
Xingyu's findings revision

\subsection{10/9}
Timeline: 
By 10/16:
\begin{itemize}
    \item The literature review
    \item The discussion
\end{itemize}

By 10/23
\begin{itemize}
    \item Method
    \item Intro and Section 3 (feminism perspective on emotion regulation revision)
\end{itemize}

By 10/30
Go over the manuscript and other emerging comments by professors.

\subsection{10/02}
why technology-supported emotion coping
emotion coping
emotion coping in carework
feminism in carework


\subsection{0821}
should we expand the scope to care work?


\subsection{0814}
2. exchange paper reading results
3. next
annotating the basic researcher gender? male-centric approach and female researcher-led  (check their online information, to check the gender ; or talk about a trend; )
screen all the paper first and get a general sense 
More about disease-related?


\subsection{0807}
the recruitment criteria/measures for the disease; 
search venues:
NORDICHI

\subsection{0730}
Is there a word that could be an alternative for emotion regulation? it advocates for the normative oppression of emotions. Emotional care sounds weird. 

Two takeaways from the feminist perspective about emotion:
Emotion Regulation experiences to live with the bizarre, intense, and uncontrollable rising feelings. 
Emotion Regulation as labor to maintain the social identity 

From the disability theory
Preserving identity
Maintaining the 

\section{lit coding}
A messy list of things to think about in literature coding. 
\begin{itemize}
    \item How do technology serve as a mediator for emotional support between and among people?
    \item How does technology understand care and the knowledge about care? Does it align with the feminist approach? \cite{bardzell_towards_2011}
    \item Who designed these care technologies? 
    \item Does technology help emotional labor? Technology can't act alone as an artifact but as an ice-breaker, an object as other toys for interpersonal emotional support \cite{theofanopoulou_exploring_2022}, and who are those human moderator? Are they females or males? What about the online moderators on peer-support groups?
    \item How does technology help with the dilemma about the disclosure and local knowledge in emotional coping? Especially in culturally-sensitive and context-aware? Is there a way for technologies to realize these without intruding on privacy?
    \item Seeking for justice in the real world is at the core of feminism. How do HCI studies reflect these?
    \item How are care and tech-mediated care different?
    \item What emotions are used for? In Orson's \cite{wu_mindshift_2024}, three emotions, boredom, stress, and inertia are three minds, used as context to be input in the LLM for persuasive message generation.
    \item What are the intentions behind emotion recognition? Is that for providing care? \cite{diberardino_anti-intentional_2023}
\end{itemize}

Other notes
\begin{itemize}
    \item Think about the non-categorical perspective and the difficulties we face in the formation of a ground truth in image annotation. How to reconcile these tensions?
\end{itemize}

Technologies for stages/needs during disease
Figure URL: https://journals.lww.com/indjem/fulltext/2018/22050/Emotional_and_Psychological_Needs_of_People_with.22.aspx

companion
general distress

crisis
after diagnosis


==> tabs/annotation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[h]
\caption{Categories of the empirical studies regarding Tools, Goals, and Roles}
\label{tab:annotation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllllllllll@{}}
 &
  \multicolumn{5}{c}{\textbf{Tools}} &
  \multicolumn{4}{c}{\textbf{Goals}} &
  \multicolumn{3}{c}{\textbf{Roles}} \\
\multicolumn{1}{c}{\textbf{Paper}} &
  \multicolumn{1}{c}{\textbf{Track}} &
  \multicolumn{1}{c}{\textbf{Tangible}} &
  \multicolumn{1}{c}{\textbf{CA}} &
  \multicolumn{1}{c}{\textbf{CSS}} &
  \multicolumn{1}{c}{\textbf{VR}} &
  \multicolumn{1}{c}{\textbf{Down}} &
  \multicolumn{1}{c}{\textbf{Up}} &
  \multicolumn{1}{c}{\textbf{Non-jud}} &
  \multicolumn{1}{c}{\textbf{Ident}} &
  \multicolumn{1}{c}{\textbf{Generator}} &
  \multicolumn{1}{c}{\textbf{Mediator}} &
  \multicolumn{1}{c}{\textbf{Nudge}} \\
\textcite{10.1145/3490149.3501326} &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3064663.3064697} &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3154862.3154929} &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3511047.3537691} &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3660244} &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3460418.3479342} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3628516.3655795} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3575879.3575997} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3130943} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/2809915.2809917} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
   &
   &
   \\
\textcite{10.1145/3411764.3445178} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3109761.3109790} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
   \\
\textcite{10.1145/3628516.3655820} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3491102.3501925} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3383313.3412244} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3421937.3421975} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3544548.3581048} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3152771.3152793} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3512939} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/2674396.2674456} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/2674396.2674453} &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3434073.3444669} &
   &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/2544104} &
   &
  \cellcolor[HTML]{FCE8B2}{\color[HTML]{9900FF} *} &
  \cellcolor[HTML]{FCE8B2}{\color[HTML]{9900FF} *} &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3173574.3174069} &
   &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.5555/3523760.3523888} &
   &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/3349537.3351907} &
   &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3491102.3502135} &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/3569484} &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3329189.3329209} &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{F4C7C3}* &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3341163.3346933} &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3381016} &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3491102.3502130} &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3325480.3325491} &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/3479561} &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
   &
   &
   \\
\textcite{10.1145/3442381.3450097} &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
\textcite{10.1145/3613904.3641922} &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3173574.3173905} &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3613904.3642761} &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3396868.3400898} &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3613904.3642123} &
   &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
   \\
\textcite{10.1145/3585088.3589381} &
   &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{F4C7C3}* &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3643834.3661570} &
   &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/2660579.2660590} &
   &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3639701.3656304} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
   \\
\textcite{10.1145/3415183} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   \\
\textcite{10.1145/3415222} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
   \\
\textcite{10.1145/3637409} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/3078072.3079742} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
  \cellcolor[HTML]{F4C7C3}* &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/3316782.3321525} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3429360.3468190} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* \\
\textcite{10.1145/3610073} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/1517744.1517804} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}* &
   \\
\textcite{10.1145/2851613.2851678} &
   &
   &
   &
  \cellcolor[HTML]{FCE8B2}* &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{B7E1CD}*
\end{tabular}%
}
\footnotesize Note: We use abbreviations in the table headings for presentation purposes. Here is the full name of the headings: Track->Emotion tracking \& management tools, Tangible-> Tangible devices, CA-> Conversational agents, CSS-> Communication support system, VR-> Virtual reality; Down-> Down-regulation goals, Up-> Up-regulation goals, Non-jud-> Non-judgmental emotion support, Ident->Identity preservation.
\end{table}

==> tabs/jiaying-tools.tex <==
\begin{table}[ht]
    \centering
    \caption{Categories and Examples of Tools }
    \label{tab:tools-example} 
    \small
    \begin{tabular}{|m{2cm}|p{11cm}|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        Category & Examples \\ \hline
        
        Virtual Reality & 
        gamified activities to enhance emotion regulation in clinical settings \cite{10.1145/3613904.3642123}. \newline
        visualizations to support emotion regulation in emergency rooms \cite{10.1145/3460418.3479342}. \newline
        reflection-based VR tools to manage negative emotions in home environments \cite{10.1145/3643834.3661570}. \newline
        technology-mediated training for cognitive reappraisal skills in social connection settings \cite{10.1145/3585088.3589381}. \\ \hline
        
        Conversational Agent& 
        language model systems for cognitive restructuring \cite{10.1145/3613904.3642761}. \newline
        crowd-powered applications to support cognitive reappraisal \cite{10.1145/3479561}. \newline
        guided chat tools based on talk therapy principles \cite{10.1145/3173574.3173905}. \newline
        anxiety management tools targeted toward college students \cite{10.1145/3396868.3400898}. \\ \hline
        
        Tangible Device & 
        devices to assist youth in coping with emotions \cite{10.1145/3491102.3502135}. \newline
        social and emotional support products for dementia care \cite{10.1145/3490149.3501326}. \newline
        AI-enabled wearable devices to track emotions \cite{10.1145/3491102.3501925}. \newline
        emotion regulation support toys for parent-child interactions \cite{10.1145/3491102.3502130,10.1145/3637409}. \newline
        affective touch devices to mitigate anxiety \cite{10.1145/3569484}. \newline
        emotion-sensing robotic companions to recognize emotions \cite{10.1145/3660244}. \newline
        portable emotion displays for children to facilitate data sharing \cite{10.1145/3628516.3655795}. \\ \hline
        
        Emotion Tracking \& Management System & 
        web-based mobile applications for emotion tracking in clinical settings \cite{10.1145/3429360.3468190}. \newline
        scalable treatment recommendation systems for health behavior management \cite{10.1145/3383313.3412244}. \newline
        data-driven mobile applications for intervention design \cite{10.1145/3421937.3421975}. \newline
        gamified apps to support routine self-management for individuals with ASD \cite{10.1145/3544548.3581048}. \newline
        wellness apps for emotion tracking among high school students \cite{10.1145/3628516.3655820}. \newline
        self-monitoring apps for negative emotion regulation in ASD populations \cite{10.1145/3329189.3329209}. \newline
        data collection tools for documenting challenging behaviors \cite{10.1145/3512939}. \\ \hline
        
        Communication Support System & 
        video-based tools to support fertility decision-making for young females \cite{10.1145/3639701.3656304}. \newline
        deep reinforcement learning agents for empathetic conversation support \cite{10.1145/3442381.3450097}. \newline
        collaborative tracking apps for birth control \cite{10.1145/3610073}. \newline
        patient advice systems for peer support in hospital settings \cite{10.1145/3415183}. \newline
        bio-data systems for heart rate sharing through messaging \cite{10.1145/3130943}. \newline
        location-based emotion annotation systems for sharing and logging \cite{huang_emotion_2015}. \\ \hline
        
    \end{tabular}
\end{table}


==> tabs/roles.tex <==
\begin{table*}[h]
\caption{Roles of technologies in carework}
\label{tab:roles}
\small
\begin{tblr}{
width = \textwidth,
colspec = {|Q[l,0.15]|Q[l,0.5]|},
hlines,
row{1} = {font=\bfseries,c,gray9},
}

Roles & Examples \\
%\textit{The technologies are designed to support the emotional coping at an individual level} 
Providing Artificial Care \newline \textit{Technologies are used as sources of affection and care.}
 & in the moment interactive, embodied technologies \cite{10.1145/3491102.3502135} \\

Facilitating Self-Guided Awareness, Reflections, Therapy \newline
\textit{Technologies are used as an assistant for emotion coping}  & Self-Guided Mental Health Interventions Through Human-Language Model Interaction \cite{10.1145/3613904.3642761}, responsive videos for emotional support during decision making of complex health decisions \cite{10.1145/3639701.3656304} \\

Merging the interpersonal communications about emotions \newline \textit{Technology-mediated emotion coping through bonding}  & \\


\end{tblr}
\end{table*}


==> tabs/tools.tex <==
\begin{table}[ht]
    \centering
    \caption{Tools and Technologies in Carework}
    \label{tab:tools-example} 
    \small
  \begin{tabular}{|m{3cm}|p{13cm}|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        Category & Examples \\ \hline
        
        Virtual Reality & 
        enhancement of emotion regulation, clinical settings, gamified activities \cite{10.1145/3613904.3642123}. \newline
        regulation of emotion, emergency room settings, visualization \cite{10.1145/3460418.3479342}. \newline
        negative emotion management and reflection, home environment \cite{10.1145/3643834.3661570}. \newline
        cognitive reappraisal skills training, technology-mediated social connection \cite{10.1145/3585088.3589381}. \\ \hline
        
        Chatbot & 
        language model-based system, cognitive restructuring \cite{10.1145/3613904.3642761}. \newline
        crowd-powered, web-based application, cognitive reappraisal\cite{10.1145/3479561}. \newline
        guided chat application, principles of talk therapy \cite{10.1145/3173574.3173905}. \newline
        anxiety management application, college students \cite{10.1145/3396868.3400898}. \\ \hline
        
        Tangible Devices & 
        assistance, emotion coping, youth  \cite{10.1145/3491102.3502135}. \newline
        products addressing social and emotional needs, dementia care \cite{10.1145/3490149.3501326}. \newline
        AI-enabled wearable device, emotion tracking \cite{10.1145/3491102.3501925}. \newline
        smart toy, emotion regulation, parent-child interactions supporter\cite{10.1145/3491102.3502130,10.1145/3637409}. \newline
        affective touch design, anxiety mitigation \cite{10.1145/3569484}. \newline
        emotion-sensing interaction, robot companion, emotion recognition \cite{10.1145/3660244}. \newline
        portable displays, children, emotion data sharing \cite{10.1145/3628516.3655795}. \\ \hline
        
        Emotion Tracking \& Management Systems & 
        emotion tracking, clinical settings, emotion regulation, web-based mobile application\cite{10.1145/3429360.3468190}. \newline
        scalable treatment recommendations, health behavior management \cite{10.1145/3383313.3412244}. \newline
        mobile application, data-driven design, interventions \cite{10.1145/3421937.3421975}. \newline
        gamified application, ASD, self-directed routines \cite{10.1145/3544548.3581048}. \newline
        wellness application,daily activities and emotion tracking, transition, high school students, mental health caring \cite{10.1145/3628516.3655820}. \newline
        ASD, negative emotion regulation,self-management, self-monitoring, mobile application\cite{10.1145/3329189.3329209}. \newline
        data collection, challenging behavior documentation \cite{10.1145/3512939}. \\ \hline
        
        Communication Support Systems & 
        Video support, fertility preservation decision-making, young females\cite{10.1145/3639701.3656304}. \newline
        deep reinforcement learning, agent, empathetic conversations support\cite{10.1145/3442381.3450097}. \newline
        application prototype, collaborative birth control tracking \cite{10.1145/3610073}. \newline
        advice system, patient, technology probe, peer support \cite{10.1145/3415183}. \newline
        heart rate sharing, messages, bio-data sharing system \cite{10.1145/3130943}. \newline
        emotion annotation, location-based mobile application, emotion regulation, sharing and logging, \cite{huang_emotion_2015}. \\ \hline
        
    \end{tabular}
\end{table}

% \begin{table}[ht]
%     \centering
%     \caption{Tools and Technologies in Carework}
%     \label{tab:tools-example} 
%     \scriptsize
%     \begin{tabular}{|m{2cm}|p{9cm}|}
%         \hline
%         \rowcolor[HTML]{EFEFEF} 
%         Category & Examples \\ \hline
        
%         VR Section & 
%         ARCADIA: Enhances emotion regulation and self-compassion, clinical settings, gamified activities \cite{10.1145/3613904.3642123}. \newline
%         Mood Worlds: Regulates emotions, in emergency room, visulization\cite{10.1145/3460418.3479342}. \newline
%         MoodShaper: Manages and reflect negative emotions, at home \cite{10.1145/3643834.3661570}. \newline
%         Cognitive reappraisal skills training, technology-mediated social connection \cite{10.1145/3585088.3589381}. \\ \hline
        
%         Chatbot & 
%         Language model-based system, cognitive restructuring \cite{10.1145/3613904.3642761} \newline
%         Crowd-powered web application, cognitive reappraisals \cite{10.1145/3479561}. \newline
%         Guided chat tool, talk therapy principles \cite{10.1145/3173574.3173905}. \newline
%         Mental Mentor: Application for managing anxiety, college students \cite{10.1145/3396868.3400898}. \\ \hline
        
%         Tangible Devices & 
%         tangible devices, youth cope with emotions \cite{10.1145/3491102.3502135}. \newline
%         VITA \& SAM: Products addressing social and emotional needs, dementia care \cite{10.1145/3490149.3501326}. \newline
%         EmoGlass: AI-enabled wearable,  emotion tracking \cite{10.1145/3491102.3501925}. \newline
%         Purrble: Smart toy, emotion regulation \& parent-child interactions \cite{10.1145/3491102.3502130,10.1145/3637409}. \newline
%         Affective touch design, mitigating anxiety \cite{10.1145/3569484}. \newline
%         Emotion-sensing interactive robot companion with emotion recognition \cite{10.1145/3660244}. \newline
%         MoodGems: Portable displays, children, sharing emotion data \cite{10.1145/3628516.3655795}. \\ \hline
        
%         Emotion Tracking \& Management systems & 
%         Tool for tracking emotions,  clinical settings \cite{10.1145/3429360.3468190}. \newline
%         Scalable treatment recommendations, health behavior management \cite{10.1145/3383313.3412244}. \newline
%         Mobile app, data-driven design, interventions \cite{10.1145/3421937.3421975}. \newline
%         RoutineAid: Gamified app, ASD, self-directed routines \cite{10.1145/3544548.3581048}. \newline
%         WellConn: Wellness application, mental health care, students \cite{10.1145/3628516.3655820}. \newline
%         Application, tracking daily activities and emotions \cite{10.1145/3628516.3655820}. \newline
%         OmniTrack: Application, ASD , monitor challenges and regulate emotions \cite{10.1145/3329189.3329209}. \newline
%         GeniAuti: Application,data collection, documenting challenging behaviors \cite{10.1145/3512939}. \\ \hline
        
%         Communication Support systems & 
%         Video, supporting fertility preservation decision-making \cite{10.1145/3639701.3656304}. \newline
%         Deep reinforcement learning agent, supporting empathetic conversations \cite{10.1145/3442381.3450097}. \newline
%         Application prototype, collaborative birth control tracking  \cite{10.1145/3610073}. \newline
%         Patient Advice System: Technology probe, peer support \cite{10.1145/3415183}. \newline
%         Application, sharing heart rates via messages \cite{10.1145/3130943}. \newline
%         Emotion Map: Encourages logging and annotating emotions \cite{huang_emotion_2015}. \\ \hline
        
%     \end{tabular}
% \end{table}


% \begin{table}[ht]
%     \centering
%     \caption{Tools of technologies in carework}
%     \label{tab:tools-example} 
%     \scriptsize
%     \begin{tabular}{|m{1.5cm}|m{1.5cm}|p{10cm}|}
%         \hline
%         \rowcolor[HTML]{EFEFEF} 
%         \multicolumn{2}{|c|}{\textbf{Tools}} & \multicolumn{1}{|c|}{\textbf{Example}} \\ \hline
%         \multicolumn{2}{|c|}{VR Section\ref{Section:VR}} & 
%         \textbf{ARCADIA} used in clinical settings, enhances users' emotion regulation and self-compassion through various gamified activities \cite{10.1145/3613904.3642123}. \newline
%         \textbf{Mood Worlds} helps regulate emotions in emergency room patients through emotional visualization \cite{10.1145/3460418.3479342}.\newline
%         \textbf{MoodShaper} allows users to manage and reflect on their negative emotions at home \cite{10.1145/3643834.3661570}.\newline
%         Design for cognitive reappraisal skills training, supporting body-based experiential learning, and providing technology-mediated social connection\cite{10.1145/3585088.3589381}.
%         \\ \hline
%         \multicolumn{2}{|c|}{Chatbot} & 
%         a language model based system supports people through various steps of cognitive restructuring\cite{10.1145/3613904.3642761}. \newline
%         a novel crowd-powered web application that provides users with cognitive reappraisals of negative thoughts\cite{10.1145/3479561}.\newline
%         an online guided chat tool enables peers to chat online using  principles of talk therapy~\cite{10.1145/3173574.3173905}.\newline
%         \textbf{Mental Mentor},an application,designed to help college students manage anxiety, particularly related to academic performance \cite{10.1145/3396868.3400898}.
%         \\ \hline
%         \multicolumn{2}{|c|}{Tangible Devices} & explores the design opportunities for tangible device to help youth cope with emotionally difficult situations in-the-moment \cite{10.1145/3491102.3502135}. \newline
%         \textbf{VITA \& SAM}: two research products that address the social and emotional needs of residents in day-to-day dementia care\cite{10.1145/3490149.3501326}.\newline
%         \textbf{EmoGlass}, an AI-enabled wearable platform for emotion tracking and management to improve emotion awareness\cite{10.1145/3491102.3501925}. \newline
%         Purrble, a smart toy focused emotion regulation intervention, facilitated parent-child interactions around emotions~\cite{10.1145/3491102.3502130,10.1145/3637409}.\newline
%         Design affective touch as a new pathway to passively mitigate in-the-moment anxiety~\cite{10.1145/3569484}.\newline
%         The prototyping of an emotion-sensing, zoomorphic interactive robot companion, including a multimodal emotion recognition framework\cite{10.1145/3660244}.\newline
%         \textbf{MoodGems},a situated, modular, and portable set of physical displays that enables children to record and share their data with their families \cite{10.1145/3628516.3655795}.
%         \\ \hline
%         \multirow{2}{1.5cm}{Online \newline Technologies \newline \textit{Interactive system for supporting emotion caring  applied in digital devices.}} & Emotion Tracking \& Management \& Interventions & 
%         a software tool for tracking and managing emotions in clinical settings, providing insights and feedback to users \cite{10.1145/3429360.3468190}.\newline
%         a viable and scalable treatment recommendations system for long-term health behavior management\cite{10.1145/3383313.3412244}.\newline
%         A mobile app that leverages data-driven design to translate evidence-based interventions~\cite{10.1145/3421937.3421975}.\newline
%         RoutineAid,gamified smartphone app, aims to help people with ASD establish and maintain “self-directed” routine structures\cite{10.1145/3544548.3581048}.\newline
%         WellConn,a wellness application aims to provide mental health care to students with mental health issues \cite{10.1145/3628516.3655820}.\newline
%         A mobile/web application that allows users to seamlessly track a wide range of daily activities and emotions together~\cite{10.1145/3628516.3655820}.\newline
%         \textbf{OmniTrack}, a digital self-tracking tool enables experiences empower adolescents to monitor challenging situations, while helping them regulate negative emotions and anxiety~\cite{10.1145/3329189.3329209}.\newline
%         \textbf{GeniAuti} is a data collection tool designed around a clinical form to document challenging behaviors~\cite{10.1145/3512939}.\newline
%         \\ \cline{2-3} 
%          & Communication Supporting & 
%          Responsive video that supports fertility preservation decision-making for cancer-diagnosed young Female Patients\cite{10.1145/3639701.3656304}.\newline
%          a deep reinforcement learning (RL) agent that learns to make sentence-level edits to support more empathy conversations \cite{10.1145/3442381.3450097}.\newline
%         a collaborative birth control tracking app prototype supports communication between users and partners~\cite{10.1145/3610073}.\newline
%          The Patient Advice System, a technology probe enable peer support in the hospital\cite{10.1145/3415183}.\newline
%          Android app that allows users to share their heart rates via messages\cite{10.1145/3130943}.\newline
%          \textbf{Emotion Map} encourages users to log and annotate their emotions based on time and location \cite{huang_emotion_2015}.
%          \\ \hline
%     \end{tabular}
% \end{table}

% ARCADIA, a VR platform used in clinical settings, enhances users' emotion regulation and self-compassion through a variety of gamified activities \cite{}. VR Mood Worlds helps regulate emotions in emergency room patients through emotional visualization \cite{}, while MoodShaper allows users to manage and reflect on their negative emotions at home \cite{}. Additionally, Alexandra Kitson \citeauthor{} have explored using VR to train adolescents in cognitive reappraisal skills. 
% Beyond information delivery, VR providing more immersive experience evokes more emotional experience and support the actual practice of skills development~\cite{}. While VR holds potential as a tool for supporting emotion regulation, its equipment requirements generally confine its use to indoor settings such as emergency rooms~\cite{}, clinics~\cite{}, and homes~\cite{}.

==> temp.tex <==




% Studies on Down-regulating Anxiety  (n=14):
% Q1. What about other "heightened" negative emotions? Current e.g., distress, stress - but what about uncertainty (cognitive), self-conscious emotions (e.g., shame / embarrasement, guilt) ; Q2. What about studies with goals to "down-regulate" and "boost positivity" but do so in an experiential & personalized manner? e.g., Zhao et al., 2022)

% Smith et al., 2021. [Flip*Doubt, Crowd-Powered Cognitive Reappraisal Systems]: Reframe negative thoughts to positive; (Anxiety & Depression assessed before vs. after or over deployment): 
% Kim et al., 2023 [RoutineAid: ...Support Daily Routines of Individuals with Autism ]:  Identified "Anxiety amplified due to a broken routine" as a Challenge via a formative study w Autism stakeholders prior to deployment of smartphone app to help manage routines and life rhythms in addressing this challenge
% Zhao et al., 2022 [Affective Touch as Immediate and Passive Wearable Intervention]: wearable "passively mitigate in-the-moment anxiety." (but via experiential intervention) "affective touch effectively mitigates state anxiety in-the-moment, but NOT the physiological stress response"


% OLD: For instance, a few design solutions aim to "calm down" users at moments of high emotionality as a prerequisite for rational thinking and further ER attempts  \cite{10.1145/3585088.3589381}.  

% NEW - MOVE TO DISCUSSION: While we acknowledge the need to calm down users at moments of high emotionality to faciliate further emotion support, we caution positioning such de-escalation as the prerequisite for rational thinking that culminates the whole ER process. Rather,  ... validation-driven approach, not merely focus on "response modulation"
%[ 112] HOW Measurement Reflects Dichotomy "to catch in-the-moment affective states of users before and after experiment to test the changes of positive affect, and reduces negative affect. "

% Slovak et al., 2023 "Relaxation training: providing support to relax/down-regulate from a baseline emotional state" 
% If key emotions related to a specific disease is anxiety / stress (high-arousal emotions, inevitably the goals would be to "down-regulate", which is not necessarily inconsistent with feminist approach?  
% Perhaps we could frame approach adopted to "down-regulate" in terms of preserving individuality in affective experiences (e.g., negative emotions can be FUNCITONAL / INFORMATIVE sometimes

%-Kitson et al. (2024) discussed 2 forms of "de-escalation" as a technique to confront the challenge of high emotionality at the "reappraisal" stage. 
% One form of de-escalation is emotion validation; (Chat-based? n = 5)
% the other one is a "GROUNDING technique...de-escalate the emotions by helping clients return to the present moment by ‘focusing on and describing tactile sensations" (Tangible, embodied toys or robots / Sensory experience, n = 

%(Kitson et al., 2024 is actually a good example of how "de-escalation" involves 
%1) validation/embracing any emotions; 
%2) guide clients thru embodied experiences of emotions?)

% Several studies aimed to personalize interventions to address diverse needs of individuals (n = 9), by gathering their unique preferences and expectations before devising interventions, and enacting affordances to aid their exploration of the "emotional self" \cite{10.1145/3316782.3321525, 10.1145/3660244}.  


CUT from Up-regulate -> sum up dichotomy
%(\textbf{Final stance before wrap up this dichotomy} is embracing experiences as a \textbf{totality} including \textbf{negative} and \textbf{positive}"?  highlight "ambivalent" emotional experiences too)
%\textbf{Maybe Goals-Dichotomy can be integrated with "How do studies understand emotions (Categorical vs. Experiential, consider temporal dynamics of emotions or not)? } --> Based on such understanding, researchers design interventions aligned with their "perceived" nature of emotions, which connotes how they can best be "regulated"? For example...
%Categorical: Negative --> Positive
%Experiential: Intangible -->  Tangible (Embodied, Able to engage with elusive / volatile changes of one's own emotions); unimodal vs. multimodal emo detection; contextual features or not
%Static vs. Dynamic - model evolution of emotions in decision support/caregiving systems, validation of temporal dynamics / "capricious" nature of emotions via peer support or reframes?

% (MOVE TO DISCUSSION) Transition from Dichotomies to ER Skills: (Transient skill development) While the two dichotomies delineated above reflect the predominant categorical (vs. experiential) understanding of emotions in extant design solutions (i.e., focus on binary ER outcomes), studies that attempted to infuse emotions' experiential qualities did not offer sustainable, self-guided support or aim to cultivate affective self-efficacy offline. (i.e., lack support for long-term skill development users can engage in independent of devices / apps) 

%\subsubsection{Emotion Regulation Goals: Support skill development} 
%(COMBINE  Emo Awareness / Reflection + Skills )
%(Differentiate studies that\textbf{ do (not) }go beyond "EmoAware" stage to \textbf{scaffold} ER)
%  Aware (Early Stage): Claimed to promote emotion awareness, mindfulness, and reflection
%  Skill (Later Stage) : 
%A limited body of work sought to foster users' ER skills beyond modifying emotional states in the moment. While the latter corrective approach reflects prevailing support for response modulation (i.e., the ER strategy to address emotions that have been fairly concretized), a few studies attempted to intervene earlier in the ER process by promoting emotion awareness and reflection. Such objectives were mostly facilitated by tangible devices or self-tracking apps, which aimed to help users identify and label their affective states in conjunction with lived experiences  \cite{10.1145/3491102.3501925, 10.1145/3429360.3468190,10.1145/3152771.3152793, 10.1145/3643834.3661570, 10.1145/3628516.3655795}.

%However, these goals were rarely carried forward in assessing the interventions' efficacy. Only three studies measured changes in ER abilities via the well established Difficulties in Emotion Regulation Scale \cite{10.1145/3643834.3661570}, user beliefs about the controllability of emotions \cite{10.1145/3491102.3502130}, as well as perceived learnability of the skill after intervention \cite{10.1145/3613904.3642761}. In addition, three studies garnered qualitative insights from user evaluation, showing their designs' potential to aid reflection and enhance awareness of emotions and negative thoughts \cite{10.1145/3628516.3655795, 10.1145/3479561,10.1145/3491102.3501925}. 

% (or did not materialize these goals through concrete measurements)

% Summary: how ER ability was measured (if indeed measured) after intervention as proxy of interventions' effectiveness) 
%  Studies that use quant ER metrics (e.g., DERS; 2 studies) to assess ER skills (short-term, not transferable)
%   !!!!! Studies that gather qual user feedback (which reveal richer insights on users' dynamic needs and desires across ER stages / mixed sentiments towards how tech mediates the salience of certain emotions in (in)opportune moments 

% !!!  WHY Response Modulation not ideal: when thoughts and feelings have been fully developed since the initial emotion-eliciting incidents. In other words, such delays in infusing support concretized the challenging emotional states, which left little room for individuals' reappraisal efforts. 

%(Q. Is Acceptance the opposite end of the spectrum for Response Modulation...or "learned helplessness" - have to accept due to failed Response Modulation, which might stem from becoming aware of one's troubling emotional states or thought patterns too late in the emotional journey, harder to intervene in the whirlwind of emotions at this stage?) 

%"emotion awareness interventions are not grounded in any specific theory of change, instead relying on the notion that improved awareness of emotions will result in better ER." \parencite{petr_slovak_designing_2023} 
%"An underlying assumption in this model is that enhanced awareness will motivate users to take a proactive role in their own stress management and/or that users will reflect on the information being provided to them and as a result of that reflection change their future behaviours"
%"What would it mean to re-design the existing reflection support to provide more direct intervention support, moving beyond simple self awareness or pattern detection?"

%66 - Cognitive reconstruction: MoodShaper: A Virtual Reality Experience to Support Managing Negative Emotions \cite{10.1145/3643834.3661570}. 
%36 - cognitive reappraisal: Kitson  Co-Designing a Virtual Reality Intervention for Supporting Cognitive Reappraisal Skills Development with Youth. 
%Kitson et al. (2024) Supporting Cognitive Reappraisal With Digital Technology- A Content Analysis and Scoping Review of Challenges, Interventions, and Future Directions


Nonetheless, most interventions in our corpus provided little support after directing users' attention to their innermost feelings. This short-circuited ER process merely left users with information about their emotions, without guiding them through  how to interpret these affective states that were mostly rendered salient to them via bio-feedback and visualization of tracked emotional data. In other words, few studies further scaffolded strategies for users to cope with the identified emotions. 




%(CBT's Overemphasis on behavioral manifestation of emotions; less about non-adaptive, more so "non-normative")
We suggest researchers to reconsider "non-adaptive" as "non-normative" reading of emotional behaviors, and avoid displacing the individual from their physical and social environments, where norms about "appropriate" emotional expressions are fostered and inscribed. 
% Researchers need to be more sensitive towards the extent to which ER goals and outcomes could be extrapolated from non-adaptive behaviors (e.g., withdrawal tendency and challenging behaviors of children with ASD at school and the elderly in residential care facilities) \cite{10.1145/3512939, 10.1145/2809915.2809917}. Such behavioral manifestation of emotions is often deemed incompatible with social expectations, and leveraged as clues to "problems" seeding intervention goals in our corpus. 
On one hand, we caution the risks of oversimplifying emotional experiences of individuals via retrospective inferences from their behaviors. This reductionism may neglect lived experiences that manifest in ways not observable by social others without shared constellation of identities, or by the machines built on biased assumptions about emotional expressions \cite{}. 

%On the other hand, we suggest steering away from attribution of responsibility solely to "emoters" themselves as they navigate challenging emotional episodes; technologies may orient social others in the care environments, including those outside of direct care relationships, to critically reflect on how they perceive and interact with the care receivers before their emotions have been concretized. This dialectical approach weaves social agents into individuals' emotional experiences; while each interaction may seem trivial, their cumulative impact holds significance for sensitive attunement with the emoters' needs for support over time.

%may foster more sensitive attunement with the emoters' needs for support by involving social agents in their emotioanl episodes



Amplify UX measures for emotion experiences}
% Studies tend to use emotion regulation goals to measure the  \cite{balaam_emotion_2019}.
The majority of studies framed UX goals in terms of serving ER goals, which position low usability and user satisfaction as barriers to realizing the potential of design solutions in ER support. However, researchers need to avoid extrapolating too far from quantitative UX metrics, as promising results on user engagement with the device or system per se do not equate to therapeutic effects that signal clinical effectiveness, nor do they account for nuanced emotional changes when technologies take on the roles of generators, mediators, or nudges in people's emotional experiences. 
% cast doubt on this approach to incorporating UX measures 

While we highlight the studies that uncovered unique design challenges within qualitative feedback \cite{10.1145/3415183}, we acknowledge the feminist principle of agnosticism about quantitative and qualitative methods, which both bear risks for unjust representation of the people \cite{bardzell_towards_2011}. Thus, we advocate for triangulating assessment of user engagement and broader user experience via self-report measures, interviews, field observations and/or behavioral analyses to enrich understanding of individuals' emotional experiences.  
% give rise to the match or mismatch between expectation and performance

Relatedly, the timing and duration of assessment need to account for the temporal dynamics of emotions while users journey through their disease management. As users' cognitive and affective needs evolve along with their symptoms, technology designs need to keenly adapt to how users orient themselves to care. In particular, users might be more engaged in intervention when their contextual needs are met, and become disengaged or fall out of touch with the intervention device when their needs have shifted. 

\paragraph{Design Implications: }
% need explanation
Researchers need to attend to contextual signals in care environments and gather user feedback over the course of design deployment. Mapping different sources of insights across timepoints may help researchers identify the design components that overlook users' evolving emotional needs, which precipitate dissatisfaction and disengagement with intervention. For instance,  user satisfaction metrics can signal overall attitudes and whether technology designs have met users' expectation; when paired with qualitative feedback, they may reveal reasons behind such user sentiment and when such "estrangement" with technologies occur. In doing so, interventions can more sensitively support the dynamics of disease management by considering the evolving roles of technologies in users' care journey. 

% not just measured at one point in time but over the course of deployment/intervention - also reflect temporal dynamics of cognitive and affective user engagement, which may map onto diff user needs (met or unmet) in their emotion coping journey / disease management journey, evolving roles of tech in supporting these needs...which tech has not caught on and adapted to given lack of signals for such evolving user needs).

% Very few studies evaluated "usability" from perspectives of Diff Stakeholders or Proxy Eval by caregivers...we advocate for juxtaposing usability issues pointed out by / or ER outcome evaluations by caregivers, providers, individuals in needs and see where the misalignment occur...
% Proxy: e.g., schools/institutions but not the receivers 
% (pros vs. cons, reality constraints/ feasibility in gaining user feedback from the affected population)...
% Other stakeholders: e.g., 1 study drew on expert reviews...; ToMtool: ease of use evaluated by 1 senior + 1 therapist, NOT child)...

% e.g., cognitive and physical burdens in using intervention device given their unique care contexts/journeys 
%- observations of cognitive + affective engagement with devices/systems
%- observations of perceived immersiveness / realism and naturalness  


XX Studies Experiential delivery and expressive therapy? - not only for down-regulation in the moment, not restricted to labs (e.g., VR, immersive), but embed within care environments - render sensory enrichment accessible and flexible for individuals, especially those in positions of less power; integrating such experiential, flexible delivery of care  into their daily routines affords them agency in choosing when and how to receive care, how to "experience" emotional care via intimate senses, and interpret the roles of technology-mediated care on their own terms)


The multifaceted nature of care provision, encompassing organization, physical labor, and emotional labor, presents complex challenges for technological interventions in caregiving. Pure emotional support is inextricably embedded within physical interactions with caregivers and institutional assistance. Technology's role in facilitating physical labor can center caregivers by freeing them from other forms of labor, enabling more meaningful communications that forge trust \cite{llubes-arria_emotional_2022}.

By distinguishing emotional labor from physical labor, t



\xingyu{Designers should notice the different power of intervention exerted by different technology. Due to the constraints of VR and wearable devices, participation becomes more controlled, and are compelled to engage in the intervention. In contrast, some technologies rely on users' self-motivation. For instance, self-reported software allows individuals to choose their level of involvement, offering them greater autonomy in the process.}

% Add studies that attempted to "allow users to document and reflect" on evolving identities

%how intersectional identities as a constellation of cultural roots, learned socio-cultural scripts play a role in how one understands and expresses their emotions (picked up by machines as "behaviors" - Often ask does this person appear "rational"? - reverse interference from their "emotional behaviors")

%As one reason why cognitive modification strategies would not be compatible with these individuals' emotional experiences?
%3.1 Emotions as Experiences 
%(CITE: Lisa) a mental representation of emotion on a particular occasion is a 
%- continuously changing stream of consciousness 
%- in which core affect evolves, interacts with, and mutually constrains construals of the psychological situation

% as commonly found in the individual-level interventions in our corpus
% echo 5.3.2 As a mediator to intervene in power dynamics
% overlook the interlaced causes of such behaviors, 
%(e.g., interlaced causes could be on part of caregivers,  environmental/structural factors, or conflicts of interest among these stakeholders; band aid, patchwork - in the moment down regulation strategies often do not uncover root cause; echo emotion coping dichotomies)

% - Overemphasis on how "emoters" display their feelings or let their difficulties in ER "slip out" via so-called  maladaptive behaviors exemplify 
% - Over-reliance on individual-level interventions (n = x); rather than attribution of responsibility solely to individuals themselves to navigate emotional episodes, 
%  not only restricted within care relationships, but experiential / interactive literacy programs as activism - change how "social others" perceive and interact with care receivers 
% prioritize prominent factors made salient by  those in greater power while neglecting the voices of the less powerful, 
% address it from the wrong angle, divorced from real needs of the people, needs are propelled by intersecting identities, left attended or attended to uninvited by social others 

% Echo 5.2.3 Identity-preserving: embed designs within care environments from inception
% Another angle to challenge emotion-reason dichotomy with critiques on "behaviorism" is to debunk the "logical causes" of emotions / challenge CBT's overemphasis on "rational thinking". Sometimes people themselves don't even know / can't pinpoint why they feel a certain way (or am I supposed to feel a certain way, permission to feel - validation approach 
% Would be a particularly arduous task for those with intersecting identities, who face various sources of oppression layered upon one another - "People express health in ways that do not dualize the body-mind-setting", debunk "inflexible cause-and-effect narratives" \cite{pendse_treatment_2022} 

%(Feminist critique on "framing of problem space" trickled down to what ends up being "measured" to purportedly benchmark effectiveness - how do we avoid perpetuating "outsider perspectives" across stages of developing and assessing tech interventions? Social science RQs tend to be framed as "what is wrong with the PERSON who is experiencing the problem" rather than what about the current "social order that makes the problem likely" 

%Convenient reliance on behavioral manifestation of emotions as clues to "problems" or intended outcomes, 
%Mislead researchers to scope / tackle a non-existent problem, or 

%\subsubsection{Amplify UX measures for emotion experiences}
% Studies tend to use emotion regulation goals to measure the  \cite{balaam_emotion_2019}.
% the mixed outcomes uncovered in our down-regulation dichotomy imply that 

Beyond CogModi
% Measures on ER outcomes perpetuate the dichotomy of rationality vs. emotion,  i.e., how the ideal ER outcomes have been operationalized in assessing effectiveness of interventions, reflecting societal expectations of --- what it means to be an individual capable of managing their own emotions. (How measures reflect what is considered "excessive" or "irrational")

\xingyu{Recognizing the limitations of labeling emotions, \textcite{grill_attitudes_2022} highlight the value of ambiguity in emotion expressions to shift the focus from treating emotions as mere information to facilitating embodied interaction~\cite{10.1145/1094562.1094570}. This approach emphasizes users' self-awareness and interpretation of their emotional experiences. Design researchers have aimed to enhance engagement with bio-data to foster shared living and knowing through human-centered approaches~\cite{10.1145/3532106.3533477}.}
\xingyu{For instance, \citeauthor{10.1145/2901790.2901850} explores how the ambiguity and emotional interpretation of clothing-based biosignal displays, which offer social cues, can help validate individuals' feelings and demonstrate emotional engagement with others. Their design incorporates "design-as-affect," allowing people to use skin conductance displays to facilitate social performances. This kind of interface enables users and those around them to collaboratively interpret and create meanings for their emotional signals. }


%  "The display’s ambiguity was valued as a prompt for reflection but also hindered participants’ attempts to feel validated. Participants sought to use their skin conductance display to help them enact social performances, such as showing emotional engagement with others."

%\xingyu{For instance, \citeauthor{10.1145/3429360.3468190}’s work emphasizes enhancing emotion awareness and self-management through self-tracking, although it is grounded in and motivated by Cognitive Behavioral Therapy}
% For example, although \citeauthor{}’s work is grounded in and motivated by Cognitive Behavioral Therapy, they emphasize enhancing emotional awareness and self-management through self-tracking. 
% should value people's lived experiences and


% Extend experiential delivery and expressive therapy from lab (e.g., VR, immersive) to users' everyday environment- render sensory enrichment accessible and flexible for individuals, especially those in positions of less power; integrating such experiential, flexible delivery of care  into their daily routines affords them agency in choosing when and how to receive care, how to "experience" emotional care via intimate senses, and interpret the roles of technology-mediated care on their own terms, e.g., same sensory experience can be used for down-regulation or merely awareness

% Shift from changing how one "thinks" about emotional events (e.g., cognitive reappraisal), to encouraging engagement with meta-emotions via bodily experiences (i.e., how one "feels" about emotions, such as frustrated at one's own anxiety, guilty about being upset). This experiential, reflexive approach can be supported by multisensory affordances of technology interventions. 

% mere act of sharing could be conceived as "care", e.g., study on sharing heart rate w/o labeling emotions, locus of interpretation of biomarkers lies in the "recipients" of the heart rate patterns and what emotional signals can be extracted from it - an attempt at evading the "mapping" issue?

% Future designs should recognize and respond to the physical manifestations of emotions to facilitate embodied interaction with the feelings of oneself and others \cite{costanza-chock_design_2020, 10.1145/1094562.1094570}. 

% For instance, (examples of "sensitive technology designs", autonomy balanced with users' unique expectations)

% Grounded upon the feminist perspective that views emotions as a source of knowledge and power rather than weakness.\cite{barrett2006emotions}, we advocate for empowering users to understand and navigate their rich spectra of emotions. 
% For instance, while anxiety and anger are often presumed to impair well-being and hinder the enactment of rational decisions, they may also heighten focus and motivate change to current circumstances \cite{}. 


In addition, our review identified a notable gap in addressing the gendered labor reality of emotional support. Feminist scholars recognize emotional support as a form of labor that plays a crucial role in fostering engagement and relationships \citep{hochschild2019managed,smriti_emotion_2024}. They highlight the often invisible and unacknowledged nature of emotional care, challenging societal expectations that women should naturally provide this care without recognition or compensation. Care provision encompasses organizational, physical, and emotional labor, which presents complex challenges for technological interventions in caregiving. Pure emotional support is inextricably embedded within physical interactions with caregivers and institutional assistance. By easing physical demands, technologies can allow caregivers to focus more on meaningful interactions that forge trust with care receivers \cite{llubes-arria_emotional_2022}.

\xingyu{Instead of directly intervening in people's emotional experiences, they aim to enhance emotional expression, awareness, and communication through various interfaces—including tangible interfaces, online applications, and VR—to address power imbalances in emotional communication. For instance, \citeauthor{10.1145/3610073} designed an application prototype to facilitate communication between users and their partners, supporting them in engaging more fully and expressing emotional support.It is noted that although some studies aim to strengthen communication between specific groups and their caregivers\cite{}, when the focus is therapeutic, the emphasis often shifts toward emotion regulation and treatment. Therefore, we recommend that future designs consider the care recipients' control over the intervention and their comfort in expressing themselves.}



%"Co-construction of the core research activities and goals…researchers and research subjects should collaboratively frame research questions".)
% Empower the "people" that we aim to extend care towards in co-constructing goals of designing technology-mediated emotion support \cite{}... Critically reflect on whose voices to account for across stages of intervention development, such as scoping research objectives and determining what methods and tools are appropriate to assess efficacy, employing or even developing measurements of emotions that are culturally grounded and honor the lived experiences of individuals and social groups that the intervention aims to support. 


Coping Dichotomy Notes
% OLD: Measures of intended ER outcomes also reflect such dichotomies
%Studies assessed positive and negative affect via PANAS pre- and post- intervention and showed 
%xx studies demonstrated reduction in emotional intensity, negative affect (e.g., anxiety, depression) over the deployment of interventions,  \cite{10.1145/3479561, 10.1145/3421937.3421975, 10.1145/3173574.3174069} but only xx studies demonstrated the efficacy of...

% NEW: Complexity in "down-regulation" as a process and an ER goal - NOT as clear cut as lower scores in PANAS, accompanied by challenges or "loopholes" in methodologies / execution? 
% --> Echo Discussion need to triangulate assessments 
% 1) measured pos neg emo but did not report in results, or measured limited emotions, approximate it with personality traits 
% 2)  did show reduction of neg emo in quant metrics, but "qualitative differences" in how such reduction occurs and why 
% 3) did reduce self-report anxiety in-situ but not Physiological Stress response

% ER SKILL-RELATED --------------

% Flip*Doubt - did reduce negative thinking, but did NOT learn or apply CR SKILLS
% "even though participants enjoyed mood boosts, occasional laughs, and even reductions in negative thinking, we observed only MINIMAL evidence that Flip*Doubt users actually \textbf{learned or applied the SKILL of cognitive reappraisal} through receiving reframes from others. Conversely, some participants described cognitive overload" 

% MoodShaper did successfully down-regulate neg emo, but NON-sig results on Awareness & Clarity subscales on SDER; only sig on Non-acceptance, Modulate 
% (echo "modification paradigm" in Discussion, band-aid, address symptoms but not root cause? What about their qual findings? Risk of VR or other immersive affordances at heightening salience of neg emo unexpectedly, or at inopportune times, or in manners that are uncontrollable by emoters?

% UNINTENDED Outcomes or Mechanisms (e.g., distraction) ----------------------------
% "Suddenly, we got to become therapists for each other (Peer Support Chat)" - both guided & unguided chats did reduce anxiety but "in qualitatively different ways", some even report trouble 
% -- Guided chats "deep": perceived as deeply valuable for gaining solutions \& insights / new perspectives but provoked UNWANTED FOCUS on TROUBLES in some cases. 
% -- Unguided chats "smooth": experienced as smooth \& easy-going, offered personal connection on shared experiences but tended toward DISTRACTION from troubles rather than emotional support.

% MoodShaper: tangible portrayal neg emo in VR "made situsations even MORE Stressful   \cite{10.1145/3643834.3661570}
% ---"negative emotions became corporeal and tangible through visual representation, exerting power over the participants. Participants frequently visualised feelings of HELPLESSSNESS & LOSS OF CONTROLby enclosing themselves within their drawings}" , "had made that situation even MORE STRESSFUL".reported UNEASE, tingling sensations, and heightened heart rates."

% Flip*Doubt - Cognitive Overload 
% ----"some people grew to RESENT this FOCUS on Negativity over time, even if the system caused them to initially develop a useful and desirable \textbf{awareness} of their negative thought patterns."


% MODALITY of Measurements -RELATED --------------
% \cite{10.1145/3173574.3174069} Huggable measured PANAS, anxiety, but did NOT report results on these; only from sentiment analysis of conversations (non sig on anxiety so chose not to report?) 
% Sentiment analysis with IBM Watson’s Tone Analyzer: "joy, agreeableness, extraversion and sadness scores were measured for each utterance sentence and were averaged for each participant’s session."
% despite increasing positivity in conversation, positivity tapered off since children actuallly felt sad towards the end bc companion robot is leaving (i.e., anticipate they would be left alone again?)

% Affective Touch as Immediate and Passive Wearable Intervention]: \cite{10.1145/3569484} 
% wearable "passively mitigate in-the-moment anxiety." (but via experiential intervention) "affective touch effectively mitigates state anxiety in-the-moment, but NOT the Physiological Stress response"



% NOTE on Irreversibility of Pos-Neg Emo: More positive affect does NOT equal to reduction in negative affect, and vice versa; might just be "cover-up" or temporary shift in attention (challenge the dichotomy, positive vs. negative emotions are NOT two ends of the spectrum
% A few studies only report on increase positive affect not decrease negative affect - by directing individuals' attention to positive feelings, at the same time ignore the negative emotions (but they are still there...just left unattended...)


Introduction}
HCI and CSCW scholars have increasingly focused on emotional wellbeing in various contexts, including workplaces, everyday life, and academic settings. Emotional work has gained particular importance in care-related domains, such as managing chronic diseases, mental health, and supporting vulnerable populations like children and older adults.
With a notable increase in studies that aim to recognize, track, and manage individuals' emotions \cite{andalibi_human_2020}, these practices often adopt the psychological framework of "emotion regulation" to develop technologies as design solutions. However, traditional approaches to emotion regulation have been criticized for their focus on modifying or suppressing emotions, reflecting a bias towards "correcting" emotional responses. This perspective fails to acknowledge the multiple sources of emotions \cite{sloan_emotion_2017}, which have been linked by some scholars to normative assumptions and even social oppression \cite{bhattacharjee_whats_2023}.

Critics argue that technologies for emotion regulation risk subjecting individual emotional experiences to surveillance and regulation through monitoring, sensing, and tracking machines \cite{boyd_automated_2023}, which intrude into people's most sensitive and private spaces \cite{choe_emotion_2023}. 

Treatment-centered research is typically based on psychological theories such as emotion regulation process model \cite{gross_antecedent-_1998} and cognitive behavioral therapy \cite{beck201960},
which may sustain the coloniality through technical design. Scholars have noted that digital tools may serve as a new vector for colonialism and oppression, advocating for justice- \cite{chordia_social_2024} and ethics-oriented research. This paradigm may contribute to stigmas around diseases and force the marginalization of certain communities by labeling them as "ill" \cite{pendse_treatment_2022}.

TRANSITION Before Jump to Feminism - 

Feminism has made foundational contributions to the social and experiential understanding of emotions, challenging biology-determined and categorical approaches. We leverage feminist perspectives on psychology and emotions to chart the dimensions of "emotional support" (as distinct from the psychological term "emotion regulation") to challenge traditionally male-dominated knowledge creation about mental health and psychological understanding of human emotions. A feminist approach to emotional support emphasizes acceptance and validation rather than correction, aligning more appropriately  with the real-world experiences of individuals facing systemic challenges \cite{hooks_feminism_2000}.

POSITIVE EXAMPLES: A growing body of work has challenged the...
JOIN POSITIVE FORCE
This work aims to reimagine technology's goals and roles in care-centered emotional support, inspired by critical reflections on the potential harms of digital tools to human feelings \cite{pendse_treatment_2022}, identities \cite{pendse_marginalization_2023}, and experiences \cite{feuston_everyday_2019}. 
% \begin{itemize}
% \item RQ1: How does feminism understand human emotion and emotion support?
% \item RQ2: What are the tools, goals, and approaches of current HCI studies on technology-mediated emotion support?
% \item RQ3: What are the implications of feminism on future technology design of emotion support?
% \end{itemize}
We conducted a systematic literature review of the ACM Digital Library, investigating the design of existing technology-mediated emotion interventions. Our analysis identified 61 relevant empirical studies, which we mapped and critically examined inspired by feminist HCI and feminist knowledge about emotion. First, we aim to identify the objectives of technology-mediated emotion intervention tools that significantly structure and influence users' understanding of and interaction with their feelings. Our analysis revealed a coping dichotomy in the emotion regulation goals of these studies. Beyond this, we also identified related user experience goals and care-centered objectives, such as non-judgmental approaches and identity preservation. 
Second, recognizing emotions as socially constructed, as per feminist understanding, we situated the technological interventions from empirical studies within the care ecosystem, encompassing the individual requiring care, informal caregivers, and health professionals and institutions. This contextual analysis uncovered three prominent roles that technologies play: directly generating artificial care, intervening in power dynamics, and nudging behavioral changes. Our study emphasizes the critical importance of contextual, culturally sensitive, and empowering approaches to emotional well-being in technological interventions.

This study emphasize the importance of contextual, culturally sensitive, and empowering approaches to emotional well-being in technological interventions. Specifically, we make the following contributions: 
\begin{itemize}
\item We critically examine "emotion regulation" practices in technological interventions, which predominantly rely on cognitive modification of human emotions. As an alternative, we propose a human-centered "emotion support" approach that validates individuals' emotional experiences, acknowledging the complex, socially constructed nature of emotions.
\item We delineate the roles technologies play within the caregiving ecosystem. Our analysis reveals the potential of these technologies to mitigate caregivers' emotional labor, preserve individuals' identities throughout their care-seeking journeys, and recalibrate power dynamics between caregivers and care receivers. This nuanced understanding paves the way for more contextually aware, culturally sensitive, and empowering approaches to emotional well-being in technological interventions.
\end{itemize}

% regulatory focus, treatment centered, standardized outcomes 
% frame certain emotional responses as problematic, to be modified

Social justice CITE
demonstrate how frameworks can help researchers
intentionally center marginalized populations, account for overlooked
harms, and provide value commitments that can guide the
research process.

This rigid perspective has been critized to minorize certain emotional experiences...


 Technologies with immersive and tactile affordances are increasingly being utilized to offer in-situ support for emotion regulation and validation, connecting real-time regulation with sensory experiences of emotions. These interventions collect sensory signals from individuals and deliver sensory feedback, facilitating experiential approaches to emotion regulation. Research has explored various technological methods to provide artificial care, with promising findings across different modalities. For instance, \textcite{10.1145/3491102.3502135} demonstrated the effectiveness of technology-enabled objects in aiding down-regulation and promoting self-compassion during heightened emotional states. Studies on artificial hugs \cite{10.1145/3341163.3346933, 10.1145/3173574.3174069} and robot touch \cite{10.1145/2544104, 10.1145/3154862.3154929, 10.1145/3569484} have shown that technology-mediated physical interactions can provide comfort and emotional support. Additionally, some studies into robot companions \cite{10.1145/3434073.3444669, 10.1145/3660244} as sources of consistent emotional stability. The affective affordances in the embodiment and interactiveness \cite{10.1145/2110363.2110398} are core for using technological sensory experiences in enhancing real-time emotional support and mental health care.


 Chatbots have shown promise in delivering therapeutic effects\cite{10.1145/3613904.3642761, 10.1145/3479561, 10.1145/3173574.3173905, 10.1145/3396868.3400898}. Powered by natural language processing (NLP), AI-based systems can generate human-like responses. As a result, researchers have developed chatbots as digital emotional support agents, grounded in counseling strategies and therapeutic theories, with studies like \cite{10.1145/3613904.3642761}. Beyond chat tools that can directly interact with users to provide emotional support \cite{10.1145/3479561, 10.1145/3396868.3400898}, some language-based AI systems can be integrated into conversations between people \cite{10.1145/3173574.3173905}, facilitating peer-to-peer emotional communication. Similarly, the system can support users in achieving cognitive restructuring and emotion regulation by editing their sentences\cite{10.1145/3613904.3642761}. Chatbots offer potential for providing real-time, language-based emotional support and treatment.

==> xingyuversion.tex <==
\subsection{Tools}

We grouped the tools for emotion coping into four main categories: Virtual Reality (VR), Chatbot, Tangible Devices and Online technology. Although some tools may blend features across categories, they are categorized based on their core functions related to emotion caring, ensuring that the focus remains on how these technologies address emotional well-being.

\input{tabs/jiaying-tools}
\subsubsection{Virtual Reality}
\label{Section:VR}
%Visual-based tools refer to technologies that provide emotion caring through visual aids or visual information. 
Four studies designed virtual reality (VR) to facilitate the emotion coping needs of users from various backgrounds including patients engaged in therapy \cite{10.1145/3613904.3642123,10.1145/3460418.3479342}, people with negative emotion \cite{10.1145/3643834.3661570}and youth \cite{10.1145/3585088.3589381}.
Typically, such deployment was combined with various therapeutic strategies including exposure therapy ~\cite{10.1145/3460418.3479342,10.1145/3613904.3642123,10.1145/3585088.3589381}, mindfulness therapy~\cite{10.1145/3613904.3642123}, and cognitive reappraisal~\cite{10.1145/3460418.3479342,10.1145/3643834.3661570,10.1145/3585088.3589381}.
 % 4 studies explore VR applied for supporting emotion regulation and expression due to its strong immersive capabilities~\cite{10.1145/3613904.3642123,10.1145/3585088.3589381,10.1145/3460418.3479342,10.1145/3643834.3661570}in various therapeutic strategies including exposure therapy ~\cite{10.1145/3460418.3479342,10.1145/3613904.3642123,10.1145/3585088.3589381}, mindfulness therapy~\cite{10.1145/3613904.3642123}, and cognitive reappraisal~\cite{10.1145/3460418.3479342,10.1145/3643834.3661570,10.1145/3585088.3589381}. 
% ARCADIA, a VR platform used in clinical settings, enhances users' emotion regulation and self-compassion through a variety of gamified activities \cite{}. VR Mood Worlds helps regulate emotions in emergency room patients through emotional visualization \cite{}, while MoodShaper allows users to manage and reflect on their negative emotions at home \cite{}. Additionally, Alexandra Kitson \citeauthor{} have explored using VR to train adolescents in cognitive reappraisal skills. 
These researchers are motivated by the unique affordances of VR, particularly its ability to quickly create environments that transcend reality, for example, \citeauthor{10.1145/3613904.3642123} built a garden, symbolizing the user's therapeutic journey, expanding the scope of therapeutic activities for patients. Studies have leveraged VR to provide immersive experiences, which are essential for evoking emotional expression~\cite{10.1145/3643834.3661570,10.1145/3460418.3479342}. This immersive quality supports both treatments led by caregivers~\cite{10.1145/3613904.3642123} and self-care practices~\cite{10.1145/3643834.3661570,10.1145/3460418.3479342}, while also facilitating the practical development of skills~\cite{10.1145/3585088.3589381}.
However, studies commonly reported limitations of VR regarding equipment requirements typically limit its use to indoor environments such as clinics~\cite{10.1145/3613904.3642123}, and homes~\cite{10.1145/3643834.3661570,10.1145/3460418.3479342}. Thus, VR is primarily used for treatment rather than for tracking.
 
% These researchers are motivated by the affordances of VR regarding A, B, C. For example, one study utilized the immersive nature of VR to [unique VR features that fit the emotion coping needs of a specific population, for example, the immersive gardening for imitated but vivid experiences. multiple examples are better since we have many VR studies.] XX studies reported positive outcomes in A, B, C . XX reported non significant results. However, some qualitative results raised concerns about ...

% \subsubsection{New VR}
% A "formula" for the tool sections. Highlight, use a third-person tone, 5 studies found; 9 studies reported; The outcomes of the studies, etc. [Easieast way: You can add these to the beginning of some of your summary]
% \begin{itemize}
%     \item How many studies.
%     \item In what care context, which population, and what emotion coping.\
%     \item How the affordances of these tools match the emotion support context.
%     \item What outcomes they found regarding this type of tool for Emotion support (pros and cons)
    
% \end{itemize}

% XX studies designed virtual reality to facilitate the emotion coping needs of users from various backgrounds including children \cite{}, people with autism \cite{}... Typically, such deployment was combined with various therapeutic strategies including exposure therapy ~\cite{10.1145/3460418.3479342,10.1145/3613904.3642123,10.1145/3585088.3589381}, mindfulness therapy~\cite{10.1145/3613904.3642123}, and cognitive reappraisal~\cite{10.1145/3460418.3479342,10.1145/3643834.3661570,10.1145/3585088.3589381}. 
% These researchers are motivated by the affordances of VR regarding A, B, C. For example, one study utilized the immersive nature of VR to [unique VR features that fit the emotion coping needs of a specific population, for example, the immersive gardening for imitated but vivid experiences. multiple examples are better since we have many VR studies.] XX studies reported positive outcomes in A, B, C . XX reported non significant results. However, some qualitative results raised concerns about ...

\subsubsection{Chatbot}
\label{Section:Chatbot}
 Chatbot have shown promise in delivering therapeutic effects\cite{10.1145/3613904.3642761, 10.1145/3479561, 10.1145/3173574.3173905, 10.1145/3396868.3400898}. Powered by natural language processing (NLP), AI-based systems can generate human-like responses. As a result, researchers have developed chatbots as digital emotional support agents, grounded in counseling strategies and therapeutic theories, with studies like \cite{10.1145/3613904.3642761}. Beyond chat tools that can directly interact with users to provide emotional support \cite{10.1145/3479561, 10.1145/3396868.3400898}, some language-based AI systems can be integrated into conversations between people \cite{10.1145/3173574.3173905}, facilitating peer-to-peer emotional communication. Similarly, the system can support users in achieving cognitive restructuring and emotion regulation by editing their sentences\cite{10.1145/3613904.3642761}. Chatbots offer potential for providing real-time, language-based emotional support and treatment.

\subsubsection{Tangible devices}
\label{Section:Tangible Devices}
\begin{figure}[h]
        \centering
        \includegraphics[width=0.75\linewidth]{figs/toyexample.png}
        \caption{Examples of Tangible Toys}
        \label{fig:toyexample}
    \end{figure}
      
Tangible devices enhance patients' emotions by influencing their physical perceptions, naturally providing support that is well-suited and connected to their current environment and circumstances. Consequently, these devices are increasingly being utilized to offer in-situ support for emotion regulation and validation, linking real-time regulation with the sensory experiences of emotions \cite{10.1145/3491102.3502135,10.1145/3490149.3501326,10.1145/3491102.3502130,10.1145/3637409,10.1145/3569484,10.1145/3660244}. Tangible devices facilitate technology-mediated physical interactions to support real-time emotional care. Compared to other tools, tangible devices are always not limited to tactile sensations; as intelligent entities, they often provide multiple forms of sensory stimulation and feedback \cite{10.1145/3569484,10.1145/3660244,10.1145/3490149.3501326}. Beyond digital interactions, they offer physical-world interaction methods.

\label{wearable devices}
\subsubsection{Wearable devices} Wearable devices is another tangible device equipped with multiple sensors. different from the tangible devices mentioned above, wearable devices primarily handle emotion tracking\cite{10.1145/3491102.3501925} and sensory providing\cite{10.1145/3569484} cooperating with software \cite{10.1145/3491102.3501925} in emotion regulation.They contribute to emotion regulation by continuously and automatically detecting and collecting users' emotional data. Thus, they can be less burdensome for users, especially those facing motivational or cognitive challenges. Recent research has shifted towards automated, multi-modal approaches to emotion detection \cite{10.1145/3491102.3501925,10.1145/3130943}, incorporating facial expressions \cite{10.1145/3491102.3501925}, speech audio \cite{10.1145/3383313.3412244}, bio-signals \cite{10.1145/3130943}and other sensing data \cite{} to map synchronized emotional changes \cite{10.1145/3383313.3412244}.  

% Due to their portability, wearable devices can provide more timely feedback and adapt to more scenarios compared to embodied toys.

\subsubsection{Emotion tracking and management systems}
Emotion tracking and management systems refer to mobile and web applications that track users' emotions and behaviors, while providing suggestions and sensory feedback, aim to support emotion regulation or improve emotional awareness to encourage self-reflection \cite{10.1145/3628516.3655820,10.1145/3329189.3329209}. 
These systems track emotions through two main methods: self-reporting and automatic detection (Section \ref{wearable devices}).
Although recognizing emotions through automated data analysis via Emotion AI can reduce the user’s burden, previous research has highlighted the ethical and social implications of applying this technology\cite{10.1145/3442188.3445939,roemmich2023emotion}. 
% Meanwhile, paradigms for understanding human emotions—many of which are adopted from other disciplines by computer scientists—often assume that AI can produce an objective 'ground truth' about emotions, however, this is challenged by researchers who argue that conceptuazlizations of what emotions are different and personalized \cite{10.1145/3442188.3445939}.
Compared to automatically emotion tracking applications, self-reporting tools allows users to define and interpret their emotions. These systems are designed to enhance emotion awareness and support self-reflection\cite{10.1145/3429360.3468190}. 
While self-report emotion applications track and record users' emotions, they typically do not intervene in emotion regulation. Instead, they support self-guided emotion management \cite{10.1145/3429360.3468190,10.1145/3544548.3581048} and provide data record to facilitate communication between users and caregiver\cite{10.1145/3628516.3655820}.


\subsubsection{Communication supporting systems}
Communication supporting systems refer to mobile and web applications enhancing interpersonal communication experiences, thereby facilitating emotional support and improving overall emotional well-being. Recognizing that emotion coping is often enacted through peer communication and can be contagious \cite{guo2020preliminary}, HCI scholars have integrated social mechanisms into technological designs to provide customized emotional support across various scenarios. The applications facilitate communication by enhancing the emotional and empathetic quality of conversations\cite{10.1145/3442381.3450097,10.1145/3610073}, providing personalized information to support decision-making\cite{10.1145/3639701.3656304}, and promoting peer support and sharing\cite{10.1145/3415183}.
%交互信息的目的， software和interactive 的优势
